OmniGaze: Reward-inspired Generalizable Gaze Estimation In The Wild

Current 3D gaze estimation methods struggle to generalize across diverse data domains, primarily due to i) the scarcity of annotated datasets, and ii) the insufficient diversity of labeled data. In this work, we present OmniGaze, a semi-supervised framework for 3D gaze estimation, which utilizes large-scale unlabeled data collected from diverse and unconstrained real-world environments to mitigate domain bias and generalize gaze estimation in the wild. First, we build a diverse collection of unlabeled facial images, varying in facial appearances, background environments, illumination conditions, head poses, and eye occlusions. In order to leverage unlabeled data spanning a broader distribution, OmniGaze adopts a standard pseudo-labeling strategy and devises a reward model to assess the reliability of pseudo labels. Beyond pseudo labels as 3D direction vectors, the reward model also incorporates visual embeddings extracted by an off-the-shelf visual encoder and semantic cues from gaze perspective generated by prompting a Multimodal Large Language Model to compute confidence scores. Then, these scores are utilized to select high-quality pseudo labels and weight them for loss computation. Extensive experiments demonstrate that OmniGaze achieves state-of-the-art performance on five datasets under both in-domain and cross-domain settings. Furthermore, we also evaluate the efficacy of OmniGaze as a scalable data engine for gaze estimation, which exhibits robust zero-shot generalization on four unseen datasets.

==> OminGaze_NeurIPS25_arxiv/figs/motivation.tex <==
\begin{figure}[!t]
    \centering
   \includegraphics[width=1.0\textwidth]{figs_o/motivation.pdf} 
   \captionsetup{font=small}
  \vspace{-10pt} \caption{\textbf{Left}: By making efficient use of large-scale diverse unlabeled datasets via reward-driven pseudo label selection, our \textsc{OminGaze} can estimate high-quality 3D gaze directions for in-the-wild images in diverse conditions, \eg, extreme head poses, varying lighting conditions, and appearance, \emph{etc}. \textbf{\textcolor{red}{Red}} and \textbf{\textcolor{yellow}{yellow}} arrows represent predictions from \textsc{OmniGaze} and base model. \textbf{Right}: our \textsc{OminGaze} achieves state-of-the-art performance on five datasets under three settings, \ie, in-domain, cross-domain, and zero-shot generalization.}
    \label{fig:motivation}
  \vspace{-24pt}
\end{figure}

==> OminGaze_NeurIPS25_arxiv/figs/overview.tex <==
\begin{figure}[!t]
    \centering
   \includegraphics[width=1.0\textwidth]{figs_o/overview.pdf}
    \put(-214.5, 164.9){\scalebox{0.65} {$\mathcal{L}^{\text{s}}$}}
    \put(-214.5, 113.5){\scalebox{0.65} {$\mathcal{L}^{\text{u}}$}}
    \put(-239, 39.6){\scalebox{0.65} {$\mathcal{L}^{\text{g}}$}}
    \put(-29, 42.4){\scriptsize {$x$}}
    \put(-38.5, 52.8){\scriptsize {$y$}}
    \put(-46.5, 38.8){\scriptsize {$z$}}
    \put(-104.9, 58.5){\scalebox{0.5} {\boldmath{$x = \cos(\psi) \cdot \sin(\theta)$}}}
    \put(-104.9, 51){\scalebox{0.5} {\boldmath{$y = \sin(\psi)$}}}
    \put(-104.8, 45.5){\scalebox{0.5} {\boldmath{$z = \cos(\psi) \cdot \cos(\theta)$}}}
    \put(-286, 58){\scalebox{0.8} {$r \ge \tau$}}
    \put(-11.5, 97){\scalebox{0.8} {$r$}}
     % \put(-91, 79.1){\scalebox{0.6} {Eq.~\ref{eq:mva_aggregate}}}
     % \put(-41, 79.1){\scalebox{0.6} {Eq.~\ref{eq:int},\ref{eq:final}}}
     \put(-316, 6){\scalebox{0.8} {(a) Training Strategy}}
      \put(-145,6){\scalebox{0.8} {(b) Reward Model as Scorer}}
   \captionsetup{font=small}
  \vspace{-18pt} \caption{\textbf{Overview of the proposed semi-supervised learning framework}. (a) \textsc{OminGaze} jointly trains on both labeled data and large-scale unlabeled data, and utilizes a reward model to select and reweight high-quality pseudo labels for unlabeled data. (b) The reward model evaluates the reliability of pseudo labels by jointly reasoning over visual appearance, scene-specific gaze descriptions, and geometric gaze directions.}
    \label{fig:overview}
  \vspace{-11pt}
\end{figure}

==> OminGaze_NeurIPS25_arxiv/figs/visual.tex <==
\begin{figure}[!t]
    \centering
   \includegraphics[width=1.0\textwidth]{figs_o/visual.pdf} 
  \vspace{-15pt}  \caption{\small{\textbf{Visual comparison results} (\S\ref{sec::zeroshot})  on four unseen datasets (\textbf{left}) and in the wild (\textbf{right}).  \textbf{\textcolor{red}{Red}} and \textbf{\textcolor{yellow}{yellow}} arrows represent gaze estimation predictions from our \textsc{OmniGaze} and base model trained only on labeled datasets. Four datasets from left to right: MPIIFaceGaze~\cite{mpiiface}, EyeDiap~\cite{eyediap}, RT-Gene~\cite{fischer2018rt}, and IVGaze~\cite{cheng2024you}. }}
    \label{fig:visual}
  \vspace{-15pt}
\end{figure}

==> OminGaze_NeurIPS25_arxiv/sec/0_abstract.tex <==
\begin{abstract}
Current 3D gaze estimation methods struggle to generalize across diverse data domains, primarily due to \textbf{i)} \textit{the scarcity of annotated datasets}, and \textbf{ii)} \textit{the insufficient diversity of labeled data}. 
In this work, we present \textsc{OmniGaze}, a semi-supervised framework for 3D gaze estimation, which utilizes large-scale unlabeled data collected from diverse and unconstrained real-world environments to mitigate domain bias and generalize gaze estimation in the wild. 
First, we build a diverse collection of unlabeled facial images, varying in facial appearances, background environments, illumination conditions, head poses, and eye occlusions. 
In order to leverage unlabeled data spanning a broader distribution, \textsc{OmniGaze} adopts a standard pseudo-labeling strategy and devises a reward model to assess the reliability of pseudo labels. 
Beyond pseudo labels as 3D direction vectors, the reward model also incorporates visual embeddings extracted by an off-the-shelf visual encoder and semantic cues from gaze perspective generated by prompting a Multimodal Large Language Model to compute confidence scores.
Then, these scores are utilized to select high-quality pseudo labels and weight them for loss computation.
Extensive experiments demonstrate that \textsc{OmniGaze} achieves state-of-the-art performance on five datasets under both in-domain and cross-domain settings. 
Furthermore, we also evaluate the efficacy of \textsc{OmniGaze} as a scalable data engine for gaze estimation, which exhibits robust zero-shot generalization on four unseen datasets.
\end{abstract}

==> OminGaze_NeurIPS25_arxiv/sec/1_introduction.tex <==
% \section{Introduction}
% % Enhancing 3D Gaze Estimation in the Wild using Weak Supervision with Gaze Following Labels  
% % motivation：泛化到真实场景是困难的由于外观、头部姿态和遮挡的变化； 3D gaze数据的有限  
% % Unigaze： 在不同的数据域泛化是困难的 利用大量的无标注数据进行自监督

% % 由于丰富多样化（外观、头部姿态和遮挡）有标注数据的缺乏 当前的方法在不同的数据域泛化是困难的。
% % 我们提出的方法旨在 在不引入额外的技术模块的情况下，高效使用大规模的无标注数据来进行鲁棒的视线估计。
% % 首先，我们通过设计一个数据引擎来收集并为大规模的无标注数据（约1.2M)自动标注伪标签。
% % 尽管如此这些伪标签中往往存在一定的噪声，此外由于标签空间连续性的特点，基于置信度的伪标签选择算法不适用了。
% % 为了充分利用这些无标注数据, 我们提出一种半监督的学习方法, 它引入了一个额外的奖励模型来预测标签的置信度、衡量其可靠性，并为未标注数据生成伪标签信息；在伪标签信息的引导下，学生模型能够可靠地利用未标注数据。


% % 介绍任务 任务意义  
% % 当前方法怎么做的 导致泛化性弱。
% % 鉴于 xxx
% \noindent\textbf{Background.} 
% 3D gaze estimation, a crucial topic in the field of nonverbal human communication understanding,  demands tracking eye movements to predict human attention. 
% As a result, 3D gaze estimation algorithms become increasingly prominent in various real-world applications, \eg, virtual reality~\cite{mania2021gaze,pai2016gazesim,patney2016towards}, human-computer interaction~\cite{choi2022kuiper,elmadjian2021gazebar}, and driver monitor systems~\cite{khan2019comprehensive,cheng2024you}.

% % 
% \noindent\textbf{Motivation.}
% Though current gaze estimation methods have achieved impressive results, they typically fine-tune on the dataset of the target domain to get competitive results, and suffer from performance decline in different domains. 
% While many methods attempt to explore cross-domain generalization in gaze estimation, they often struggle due to impoverished training data, which are collected in specific environmental conditions and have restricted gaze distributions.
% Given the cross-domain generalization ability of foundation models in various downstream scenarios via the scaling law, the following questions naturally arise: 
% {\ding{182}} \textit{Is it feasible for gaze estimation algorithms to achieve a similar level of generalization, \ie, training a foundation model to estimate gaze direction across diverse data domains?}

% \noindent\textbf{Data Engine.}
% This question {\ding{182}} motivates us to build a foundation model capable of \textit{producing high-quality gaze directions under any circumstances from the perspective of dataset scaling-up}. 
% % 首先 获得有标注数据是困难 并且diverse有限。
% Traditionally, acquiring labeled 3D gaze data typically requires specialized hardware such as infrared eye trackers and head pose tracking systems, which is costly, time-consuming, and typically constrained to limited environmental conditions. Thus we collect large-scale unlabeled data, and further develop a data engine to automatically generate 3D gaze annotations for unlabeled images. Compared with publicly labeled 3D gaze data, our used unlabeled face images exhibit two advantages: \textbf{i)} \textit{High diversity}: face images provide a significantly higher level of diversity regarding facial appearance, lighting conditions, and head poses; \textbf{ii)} \textit{easy to annotate}: We can simply use a well-trained gaze estimation model to assign 3D gaze labels for unlabeled images, which only takes a feedforward step. We collect 1.5M diverse images from 7 datasets, \eg, xxx, xxx, and xxx. We use their raw unlabeled images without any form of labels. Then, in order to provide a reliable annotation tool for our unlabeled images, we make use of 1M labeled images from existing 3D gaze datasets to train a teacher model. The pseudo labels of unlabeled images are then automatically annotated and jointly learned with labeled images in a self-training manner.

% \noindent\textbf{Methodology.}
% Though unlabeled images offer several compelling advantages, it is still non-trivial to unlock the potential of large-scale unlabeled data while accommodating the unique characteristics of gaze estimation. This naturally raises the following questions: {\ding{183}} \textit{What are the factors influencing the positive use of pseudo gaze labels from unlabeled images?} {\ding{184}} \textit{How can we address these challenges?}

% Driven by question {\ding{183}}, we find that certain pseudo-labels can be severely incorrect during training due to the limited generalization ability of the teacher model. If we directly utilize pseudo labels from a previously learned teacher model for subsequent training, the conformance-biased information in the preceding epochs could increase confidence in erroneous predictions and eventually lead to poor performance of the student model.
% Accordingly, many existing efforts utilize confidence-based pseudo-label evaluation strategies to select high-quality pseudo labels, thus reducing the hidden noise.
% However, these algorithms are designed for classification tasks but are inapplicable for gaze estimation, which is a regression task.  \textit{Different from} classification, the output gaze labels in gaze estimation are continuous and lack confidence information, making it more challenging to assess the reliability of pseudo labels.

% As a response to question {\ding{184}}, we develop \textsc{OmniGaze}, a semi-supervised learning framework, which make efficient use of large-scale unlabeled face data for generalizable gaze estimation in the wild.
% \textsc{OmniGaze} introduces an additional rewarder that predicts confidence scores based on 3D gaze pseudo labels and corresponding unlabeled data to measure its reliability. 
% Concretely, \textbf{for the unlabeled data part}, given a full-face image with specified gaze information, an LLM is queried to generate descriptive gaze-related captions. Then, our rewarder integrates full-face visual features and such gaze-related descriptions into a robust multimodal gaze representation, thus allowing the rewarder to reason over both visual appearance and semantic context. 
% \textbf{For the pseudo-label part}, we interpolate each gaze label into a 3D gaze direction vector, which provides a geometry-aware formulation that better reflects gaze behaviors.
% Then, the rewarder models the complicated interplay between multi-model gaze features and gaze labels via cross-attention to produce initial confidence scores.
% Such a design allows the rewarder to capture semantic consistency between textual context, and gaze direction.
% To further strengthen the evaluation capability of the rewarder, we combine initial confidence scores and similarity scores between the student model prediction and the pseudo-label to obtain final confidence scores, yielding a holistic and reliable measure of pseudo-label quality. With the assistance of pseudo-label information provided by the rewarder, the student model filters out unreliable pseudo labels and reweights the importance of different high-quality samples via confidence scores. 
% Finally, to establish a loop for mutual boosting between above rewarder-inspired gaze estimation and rewarder training,  we devise an online update strategy to facilitate the continual evolving of pseudo labels during gaze estimation learning.

% \noindent\textbf{Experiments.}

% \noindent\textbf{Contributions.}
% Our contributions are summarized as follows:
% \begin{itemize}[leftmargin=*]
% \item \textbf{Generalizable Gaze Estimation in the Wild}: We present \textsc{OmniGaze}, a generalizable gaze estimation model that estimates high-quality 3D gaze directions under any circumstances via efficient use of diverse and large-scale unlabeled face images. 
% \item \textbf{Unleashing the Power of Large-scale Unlabeled Data}: We develop a data engine to collect and automatically annotate large-scale and diverse unlabeled face data, which provides a significantly high level of data diversity and addresses the data scarcity issue.
% \item \textbf{Intelligent High-quality Pseudo Label Selection}: \textsc{OmniGaze} introduce a confidence evaluator that predicts reliable scores via jointly reasoning over full-face visual embeddings, scene-specific gaze descriptions, and geometry-aware 3D gaze vectors, so as to evaluate and filter out high-quality pseudo gaze labels.
% %Our model achieves comparable or even more favorable zero-shot results to prior works fine-tuned on a target domain. Further, it outperforms SOTA methods under within- and cross-dataset settings.



% %To reliably make use of unlabeled data, we utilize an additional rewarder model to evaluate pseudo-label qualities and intelligently select a subset of them to reduce the hidden noise.

% \end{itemize}
% \section{Introduction}
% Eye gaze provides human with a means for evaluating an individual's interest in their internal and external environments~\cite{emery2000eyes}, which is subtle but informative. 
% 3D gaze estimation, as a crucial topic in the field of gaze signal analysis, aims to directly predict gaze direction from face images, which serves as the foundational representation in various applications, such as virtual reality~\cite{mania2021gaze,pai2016gazesim,patney2016towards}, human-computer interaction~\cite{choi2022kuiper,elmadjian2021gazebar}, medical diagnosis~\cite{chang2021computational,perochon2023early}, and driver monitor systems~\cite{khan2019comprehensive,cheng2024you}.
%  \input{figs/motivation}

% Due to the variants of subject appearance, background environments, image quality, shooting angle and illumination across existing datasets~\cite{eth,gaze360,gazecapture,eyediap}, the performance of gaze estimation methods trained on a single dataset suffer from performance degradation when testing on new, unseen datasets.  
% This limitation motivates recent research~\cite{gaze360,wang2019generalizing,liu2021generalizing,wang2022contrastive,bao2022generalizing,hisadome2024rotation,cheng2022puregaze,xu2023learning} to focus on cross-domain generalization for gaze estimation, seeking to bridge inter-dataset discrepancies. 
% Though effective, these methods are still constrained by the limited diversity of labeled training data, constraining their applicability for real-world applications. 
% In contrast, enormous face images can be easily accessed by crawling from Internet~\cite{CASIA-WebFace} or synthetic generation using generative models~\cite{FaceSynthetics}.

% To generalize gaze estimation with large-scale unlabeled face datasets, there are two main strands of research: \textit{weakly supervised learning} and \textit{unsupervised learning}. 
% Regarding to \textit{weakly supervised learning}, previous works enhance 3D gaze estimation with weak social gaze interaction labels (\eg, mutual-gaze~\cite{kothari2021weakly} and gaze-following~\cite{vuillecard2025enhancing}), while~\cite{ververas20243dgazenet} generates gaze pseudo-annotations by leveraging 3D eye region geometry.
% However, their effectiveness is constrained by reliance on labeled datasets from gaze-related domains.
% In the context of unsupervised learning, \textit{self-supervised pre-training} stands out as the leading paradigm, which endeavors to learn a robust gaze representation via well-designed pretext tasks, \eg, eye-consistent image reconstruction~\cite{sun2021cross,bao2024unsupervised}, masked image restoration~\cite{qin2025unigaze} and gaze redirection~\cite{yu2020unsupervised}. 
% Nevertheless, these pretext tasks exhibit weak semantic relevance to gaze estimation, resulting in inefficient utilization of unlabeled face images.

% In light of these limitations, we find that there remains a notable void for semi-supervised frameworks capable of effectively harnessing both labeled data and large-scale unlabeled datasets in the gaze estimation community.
% Then, we propose \textsc{OmniGaze}, a semi-supervised learning framework, which employs a pseudo-labeling strategy to effectively generalize gaze estimation in the wild with large-scale, unlabeled face datasets. 
% Concretely, we first leverage labeled images from existing 3D gaze datasets to train an initial teacher model, and then develop a data engine to automatically annotate pseudo labels for unlabeled face datasets from diverse domains.
% To mitigate the confirmation bias of noisy pseudo labels, we further select high-quality samples via a pseudo-labeling assessment strategy, and jointly learn the student model with filtered pseudo-labeled and labeled images. %in a self-training manner.   

% Though many existing efforts utilize dynamic or hand-crafted threshold-based pseudo-labeling strategies to filter out low-quality pseudo-labels, they are specifically tailored for classification tasks and are inapplicable for 3D gaze estimation, as probabilistic uncertainty measures cannot be derived from the regression outputs.
% Inspired by the recent success of Reinforcement Learning from Human Feedback (RLHF) in modeling nuanced human preferences for complex tasks, \textsc{OmniGaze} devises a reward model, which serves as a proxy for human-like judgments to assess the reliability of gaze pseudo labels.
% \textit{Different} from previous methods relying on handcrafted heuristics or static uncertainty metrics, our reward model jointly reasons over visual appearance, semantic gaze context and geometric gaze direction to predict confidence scores, which assesses gaze behaviors based on multiple sources of prior knowledge like humans.
% \textbf{For the visual part},  our reward model queries an MLLM with the full-face image and textual prompt to generate \textit{scene-specific gaze descriptions}.
% Then it integrates full-face visual features and such gaze-related descriptions into a robust multi-modal gaze representation, thus dynamically attending to relevant gaze cues when interpreting visual features.
% Beyond gaze semantic grounding, \textbf{for the pseudo-label part}, our reward model interpolates each pseudo gaze label into a 3D gaze direction vector, which provides a geometry-aware formulation that better reflects gaze behaviors. We further model the complicated interplay between multi-model gaze features and gaze labels via cross-attention to produce confidence scores.
% \textsc{OmniGaze} regards these confidence scores as preference signals to filter out unreliable pseudo labels and reweight the importance of different high-quality samples during the student model training.
% Finally, to establish a loop for mutual boosting between the above reward-inspired gaze estimation and reward model training,  we devise a pseudo-label update strategy to facilitate the continual evolution of pseudo labels during gaze estimation learning. This iterative feedback loop enables \textsc{OmniGaze} to progressively improve both its gaze estimation and pseudo-labeling performance.


% To fuel the proposed semi-supervised data engine, we curate a diverse collection of unlabeled face images from six publicly available sources, exhibiting wide variability in terms of facial appearance, lighting conditions, head poses, imaging environments, \emph{etc} (Table~\ref{tab:datasets}). Through embracing scaling up data as well as effective reward-inspired pseudo label selection, our \textsc{OmniGaze} surpasses all top-leading solutions on five datasets under both in-domain and cross-domain settings (\S\ref{sec::in_cross}).
% Furthermore, we demonstrate the efficacy of \textsc{OmniGaze} as a scalable data engine for generating
% reliable gaze annotations for face images under diverse conditions. Without any fine-tuning, \textsc{OmniGaze} exhibits robust zero-shot generalization across four unseen datasets, evidencing its great potential for deployment in wild-scene applications (\S\ref{sec::zeroshot}).

%  \textsc{OmniGaze} makes three main contributions to the gaze estimation community: \textbf{First}, \textbf{\textit{generalizable gaze estimation in the wild}}: We present \textsc{OmniGaze}, a powerful semi-supervised gaze estimation framework, that estimates high-quality 3D gaze directions under diverse real-world conditions via effectively harnessing both labeled data and large-scale unlabeled datasets. \textbf{Second}, \textbf{\textit{reward-driven pseudo Label selection and reweighting}}: \textsc{OmniGaze} devises a reward model that predicts reliable scores via jointly reasoning over full-face visual embeddings, scene-specific gaze descriptions, and geometry-aware 3D gaze vectors, so as to select and reweight high-quality pseudo gaze labels. The reward model mimics human-like judgment by integrating multiple sources of prior knowledge when evaluating gaze behaviors. \textbf{Third}, better \textbf{\textit{generalization}}: \textsc{OmniGaze} outperforms SOTA methods under with-domian, cross-domain and zero-shot settings, demonstrating its great potential as a generalized gaze estimator and automatic data engine.

% Specifically, we curate a diverse collection of unlabeled facial images exhibiting wide variability in terms of facial appearance, lighting conditions, and head poses, and further develop a data engine to automatically generate 3D gaze annotations for these unlabeled images, enabling data scaling-up to an arbitrary scale.
%  In order to provide a reliable annotation tool for our unlabeled images, we make use of 0.9M labeled images from existing 3D gaze datasets to train an initial teacher model. The unlabeled facial images are then automatically annotated and jointly learned with labeled images in a self-training manner.
%  \input{figs/motivation}

%  Though unlabeled facial images offer several compelling advantages, there exists noisy pseudo gaze labels due to the inherent domain bias of labeled data. Such noisy gaze labels introduce misleading supervisory signals, causing the model to learn incorrect visual-gaze association. 
%  Accordingly, many existing efforts utilize dynamic or hand-crafted threshold-based pseudo-labeling strategies to filter out low-quality samples.
%  Nevertheless, they are specifically tailored for classification tasks and are inapplicable for 3D gaze estimation, as probabilistic uncertainty measures cannot be derived from the regression outputs.
% \textsc{OmniGaze} introduces an additional rewarder that predicts confidence scores based on 3D gaze pseudo labels and corresponding unlabeled data to measure its reliability. 
% Concretely, \textbf{for the unlabeled data part}, given a full-face image with specified gaze information, an LLM is queried to generate descriptive gaze-related captions. Then, our rewarder integrates full-face visual features and such gaze-related descriptions into a robust multimodal gaze representation, thus allowing the rewarder to reason over both visual appearance and semantic context. 
% \textbf{For the pseudo-label part}, we interpolate each gaze label into a 3D gaze direction vector, which provides a geometry-aware formulation that better reflects gaze behaviors.
% Then, the rewarder models the complicated interplay between multi-model gaze features and gaze labels via cross-attention to produce initial confidence scores.
% Such a design allows the rewarder to capture semantic consistency between textual context, and gaze direction.
% To further strengthen the evaluation capability of the rewarder, we combine initial confidence scores and similarity scores between the student model prediction and the pseudo-label to obtain final confidence scores, yielding a holistic and reliable measure of pseudo-label quality. With the assistance of pseudo-label information provided by the rewarder, the student model filters out unreliable pseudo labels and reweights the importance of different high-quality samples via confidence scores. 
% Finally, to establish a loop for mutual boosting between above rewarder-inspired gaze estimation and rewarder training,  we devise an online update strategy to facilitate the continual evolving of pseudo labels during gaze estimation learning.


% \textcolor{red}{[pipeline]}

% \textcolor{red}{[rewarder]}

% \textcolor{red}{[multi-modal]}




% \noindent\textbf{Experiments.}
% Our contributions are summarized as follows:
% \begin{itemize}[leftmargin=*]
% \item \textbf{Generalizable Gaze Estimation in the Wild}: We present \textsc{OmniGaze}, a generalizable gaze estimation model that estimates high-quality 3D gaze directions under any circumstances via efficient use of diverse and large-scale unlabeled face images. 
% \item \textbf{Unleashing the Power of Large-scale Unlabeled Data}: We develop a data engine to collect and automatically annotate large-scale and diverse unlabeled face data, which provides a significantly high level of data diversity and addresses the data scarcity issue.
% \item \textbf{Intelligent High-quality Pseudo Label Selection}: \textsc{OmniGaze} introduce a confidence evaluator that predicts reliable scores via jointly reasoning over full-face visual embeddings, scene-specific gaze descriptions, and geometry-aware 3D gaze vectors, so as to evaluate and filter out high-quality pseudo gaze labels.
% %Our model achieves comparable or even more favorable zero-shot results to prior works fine-tuned on a target domain. Further, it outperforms SOTA methods under within- and cross-dataset settings.



% %To reliably make use of unlabeled data, we utilize an additional rewarder model to evaluate pseudo-label qualities and intelligently select a subset of them to reduce the hidden noise.

% \end{itemize}


\section{Introduction}
Eye gaze provides human with a means for evaluating an individual's interest in their internal and external environments~\cite{emery2000eyes,fan2019understanding}, which is subtle but informative. 
3D gaze estimation, as a crucial topic in the field of gaze signal analysis, aims to directly predict gaze direction from face images, which serves as the foundational representation in various applications, such as virtual reality~\cite{mania2021gaze,pai2016gazesim,patney2016towards}, human-computer interaction~\cite{choi2022kuiper,elmadjian2021gazebar,andrist2014conversational}, medical diagnosis~\cite{chang2021computational,perochon2023early}, and driver monitor systems~\cite{khan2019comprehensive,cheng2024you}.

\input{figs/motivation}

Due to the variants of subject appearance, background environments, image quality, shooting angle and illumination across existing datasets~\cite{eth,gaze360,gazecapture,eyediap}, the performance of gaze estimation methods~\cite{wang2023gazecaps,o2022self} trained on a single dataset suffer from performance degradation when testing on new, unseen datasets.  
This limitation motivates recent research~\cite{lee2022latentgaze,cai2023source,qin2022learning,wang2022contrastive,bao2022generalizing,hisadome2024rotation,cheng2022puregaze,xu2023learning} to focus on cross-domain generalization for gaze estimation, seeking to bridge inter-dataset discrepancies. 
Though effective, these methods are still constrained by the limited diversity of labeled training data, restricting their applicability for real-world applications. 
In contrast, enormous face images can be easily accessed by crawling from Internet~\cite{CASIA-WebFace} or synthetic generation using generative models~\cite{FaceSynthetics}.

To generalize gaze estimation with large-scale unlabeled face datasets, there are two main strands of research: weakly supervised learning and unsupervised learning. 
Regarding to weakly supervised learning, previous works enhance 3D gaze estimation with weak social gaze interaction labels (\eg, mutual-gaze~\cite{kothari2021weakly} and gaze-following~\cite{vuillecard2025enhancing}), while~\cite{ververas20243dgazenet} generates gaze pseudo-annotations by leveraging 3D eye region geometry.
However, their effectiveness is constrained by reliance on labeled datasets from gaze-related domains.
In the context of unsupervised learning, self-supervised pre-training stands out as the leading paradigm, which endeavors to learn a robust gaze representation via well-designed pretext tasks, \eg, eye-consistent image reconstruction~\cite{sun2021cross,bao2024unsupervised,wang2024bootstrap}, masked image restoration~\cite{qin2025unigaze} and gaze redirection~\cite{yu2020unsupervised}. 
Nevertheless, these pretext tasks exhibit weak semantic relevance to gaze estimation, resulting in inefficient utilization of unlabeled face images.

In light of these limitations, we find that there remains a notable void for semi-supervised frameworks capable of effectively harnessing both labeled data and large-scale unlabeled datasets in the gaze estimation community.
Then, we propose \textsc{OmniGaze}, a semi-supervised learning framework~(\cf~Fig.~\ref{fig:motivation}), which employs a pseudo-labeling strategy to generalize gaze estimation in the wild with large-scale unlabeled face datasets.
% Concretely, \textsc{OmniGaze} adopts a three-stage training strategy: 
% Typically, SSL adopts a three-stage training strategy:
Concretely, \textsc{OmniGaze} implements a standard SSL three-phase training protocol: 
\textbf{i)} a teacher model is trained via supervised learning on annotated datasets;
\textbf{ii)} this model is utilized to generate pseudo-labels for unlabeled samples and high-quality instances are selected to enhance training data;
\textbf{iii)} a generalized student model is optimized by integrating both annotated and pseudo-labeled data.
However, applying this strategy to 3D gaze estimation is confronted with three critical challenges:  {\ding{182}} existing threshold-based pseudo-labeling methods~\cite{zhou2010semi,xie2020self,kim2022conmatch}, specifically tailored for classification tasks, are \textit{inapplicable for regression output}; 
{\ding{183}} pseudo-labels generated by a teacher model trained on labeled datasets with limited diversity suffer from domain bias~\cite{yalniz2019billion}, which leads to \textit{difficulty in utilizing the pseudo labels};
{\ding{184}} learning robust gaze representations demands training data with rich diversity~\cite{yang2024depth,vuillecard2025enhancing,qin2025unigaze}  to \textit{capture the wide variability across individuals}.

Faced with challenge {\ding{182}}, \textsc{OmniGaze} devises a dedicated reward model that utilizes unlabeled images paired with pseudo labels to assess the reliability of these pseudo labels. 
To learn reliable reward scores, we propose two advancements: 
\textbf{i)} Each pseudo gaze label is interpolated into a 3D gaze direction vector, thereby enabling a geometry-aware representation and enhancing alignment with natural gaze behaviors;
\textbf{ii)} To harness the enormous knowledge stored in large-scale pretrained language models, we extract visual embeddings of unlabeled images via an off-the-shelf visual encoder and define a prompt to guide the Multimodal Large Language Model to generate \textit{scene-specific gaze descriptions} for unlabeled images;
These linguistic descriptions are encoded via the text encoder of CLIP and combined with visual features to construct a multi-modal gaze representation.
Thus, the reward model can capture the nuanced nature of gaze for robust confidence assessments.

As a response to challenge {\ding{183}}, \textsc{OmniGaze} adopt two strategies: 
\textbf{i)} utilize confidence scores to filter out unreliable pseudo labels and reweight the importance of different high-quality samples for loss computation;
\textbf{ii)} establish a loop for mutual boosting between the student model and reward model training, enabling continuous refinement of pseudo labels to progressively enhance both gaze estimation accuracy and pseudo-label quality in \textsc{OmniGaze}.

To tackle challenge {\ding{184}} and fuel the proposed semi-supervised data engine, we curate a diverse collection of unlabeled face images from six publicly available sources, exhibiting wide variability in terms of facial appearance, lighting conditions, head poses, imaging environments, \emph{etc} (Table~\ref{tab:datasets}).

Through embracing scaling up data as well as effective reward-inspired pseudo label selection, our \textsc{OmniGaze} surpasses all top-leading solutions on five datasets under both in-domain and cross-domain settings (\S\ref{sec::in_cross}).
Furthermore, we demonstrate the efficacy of \textsc{OmniGaze} as a scalable data engine for generating reliable gaze annotations for facial images under diverse conditions. Without any fine-tuning, \textsc{OmniGaze} exhibits robust zero-shot generalization across four unseen datasets, evidencing its great potential for deployment in wild-scene applications (\S\ref{sec::zeroshot}).

==> OminGaze_NeurIPS25_arxiv/sec/2_relatedwork.tex <==
%\clearpage
\section{Related Work}
% 最早期只是利用几何模型
% 早期的方法只使用卷积回归    
% 出现cnn架构  一开始只用eye后来开始用full face
%出现trasnformer架构

% \noindent\textbf{Appearance-based Gaze Estimation.} 
% Appearance-based gaze estimation aims to regress 3D gaze from 2D facial images captured by web cameras. 
% Early methods develop their algorithm using scene-restricted datasets and attempt to enhance generalizability through strategies such as extracting gaze-correlated facial features~\cite{schneider2014manifold,gazecapture,zhang2017s,fischer2018rt} or integrating geometric constraints~\cite{zhu2017monocular,park2018deep,ranjan2018light}.
% Though effective enough for certain subjects, they suffer from performance degradation in unconstrained environments, \eg, free head motion and profile faces of subjects positioned further from the camera.
% To track this issue, subsequent studies endeavor to construct datasets~\cite{eth,gaze360,gazecapture,eyediap} for gaze estimation in more physically unconstrained settings. 
% Though they employed various methods to simulate real-world scenarios, such as using panoramic cameras to record multiple participants at once~\cite{gaze360} or multi-view photogrammetry to simulate gaze variations under extreme head poses~\cite{eth}, these approaches still rely on pre-defined assumptions that inherently simplify real-world complexity, and remain difficult to scale compared to web-crawled~\cite{CASIA-WebFace}, crowd-sourced~\cite{gazecapture} or synthetic data~\cite{FaceSynthetics}.


% % \noindent\textbf{Generalized Gaze Estimation.} 
% \noindent\textbf{Cross-Domain Gaze Estimation.} 
% The scarcity of diverse \textit{labeled training data} in appearance-based gaze estimation leads current fully-supervised methods to achieve strong \textit{within-domain} performance but suffer from poor generalization in \textit{cross-domain} scenarios.
% % , limiting their applicability for real-world applications. 
% % Due to the limited diversity of annotated datasets, methods trained on them often suffer from performance degradation when tested on different domains.
% % To address this challenge, recent efforts for generalized gaze estimation can be categorized into three paradigms: domain adaptation, domain generalization, and unsupervised representation learning. 
% To address this challenge, recent efforts for gaze estimation can be categorized into two paradigms: domain adaptation and domain generalization.
% Domain adaptation approaches primarily try to minimize the domain discrepancy between source domain and known target domain by, \eg, adversarial learning~\cite{gaze360,wang2019generalizing}, collaborative learning~\cite{liu2021generalizing}, contrastive learning~\cite{wang2022contrastive}, and consistency learning~\cite{bao2022generalizing,hisadome2024rotation}. 
% In contrast, recent endeavors in domain generalization address a more realistic scenario without access to target samples, focusing on learning domain-invariant features through methods, \eg, self-adversarial learning to preserve gaze information~\cite{cheng2022puregaze} or data augmentation based on gaze-irrelevant factors~\cite{xu2023learning}. 
% % As another line of research in generalized gaze estimation, some methods endeavor to learn a robust gaze representation by utilizing enormous unlabeled data in an unsupervised manner via well-designed pretext tasks, \eg, eye-consistent image reconstruction~\cite{sun2021cross,bao2024unsupervised} and gaze redirection~\cite{yu2020unsupervised}.
% However, given the inherent diversity of facial images (\eg, illumination, head orientation, and eye occlusion variations), these methods remain constrained by their reliance on the coverage of labeled source-domain data, which hinders their performance in the unconstrained real-world environments.



% % the performance for cross-domain gaze estimation methods hinges on the coverage of labeled source-domain diversity

% \noindent\textbf{Generalizing Gaze Estimation with Large-Scale Facial Datasets.} 
% The increasing availability of other annotated face-related datasets and enormous web-crawled or synthetic facial images has driven a rising trend to generalize gaze estimation with large-scale weakly-labeled or unlabeled data.
% % With regarding to weakly-labeled data, Kothari et al.~\cite{kothari2021weakly} derive viable 3D gaze supervision from weak mutual-gaze labels, while Vuillecard et al.~\cite{vuillecard2025enhancing} enhance 3D gaze estimation with diverse 2D gaze-following data. 
% % Parallel to these efforts, Ververas et al.~\cite{ververas20243dgazenet} create a large-scale dataset of diverse faces with gaze pseudo-annotations generated by leveraging 3D eye region geometry. 
% With regard to weakly-labeled data, certain methods enhance 3D gaze estimation with weak social interaction labels, \eg, mutual-gaze~\cite{kothari2021weakly} and gaze-following~\cite{ververas20243dgazenet}, while \cite{ververas20243dgazenet} creates a large-scale dataset with gaze pseudo-annotations generated by leveraging 3D eye region geometry. 
% To leverage unlabeled data for gaze estimation, \textit{self-supervised pre-training} stand out as the leading paradigm, which endeavors to learn a robust gaze representation via well-designed pretext tasks, \eg, eye-consistent image reconstruction~\cite{sun2021cross,bao2024unsupervised}, masked image restoration~\cite{qin2025unigaze} and gaze redirection~\cite{yu2020unsupervised}.  
% Though prior works partially alleviate the label shortage issue in 3D gaze estimation, the absence of a semi-supervised framework capable of effectively harnessing both limited labeled data and large-scale unlabeled datasets leaves a notable void in the gaze estimation community. 


% \noindent\textbf{Leveraging Large-scale Unlabeled Data.} 
% How to make use of large-scale unlabeled or pseudo-labeled data has become a significant trend to alleviate the labeled data scarcity and improve model generalization in various computer vision applications. In terms of different strategies that harness unlabeled data, \textit{self-supervised pre-training} and \textit{semi-supervised learning} (SSL) are two dominant paradigms. \textbf{i)} \textit{Self-supervised pre-training} methods exploit the inherent structure of unlabeled data to learn useful visual representation by various unsupervised techniques, \eg, contrastive learning and generative learning. Contrastive learning, as the most compelling method for self-supervised pre-training, typically regards the augmented views from the same image as positive pair and different images as negative pairs, so as to learn meaningful representations in a discriminative manner. Additionally, generative methods, particularly those involving autoencoder and autoregressive modeling, typically learn latent semantic representations during pre-training with a pre-designed task, \ie, reconstructing the masked input. These self-supervised pre-training methods have achieved impressive improvement in in a wide variety of downstream tasks, such as xxx and xxx. \textbf{ii)} Recently, SSL approaches have witnessed phenomenal growth to improve model performance, evident through extensive research. Pseudo labels and consistency regularization are two major strategies for SSL. Pseudo label methods exploit the information of unlabeled data with limited labeled data in a self-training pipeline, \ie, producing pseudo labels for unlabeled samples and jointly training models with labeled data and pseudo labels. Specifically, many methods make full use of pre-trained strong teacher models to generate high-quality pseudo labels. In addition, to select high-quality pseudo labels for SSL, fixed or dynamic threshold-based pseudo labeling selection strategies are adopted. 


\noindent\textbf{Appearance-based Gaze Estimation.} 
Appearance-based gaze estimation aims to regress 3D gaze from 2D face images captured by web cameras. 
Early methods develop their algorithm using scene-restricted datasets and attempt to enhance generalizability through strategies such as extracting gaze-correlated face features~\cite{schneider2014manifold,gazecapture,zhang2017s,fischer2018rt} or integrating geometric constraints~\cite{zhu2017monocular,park2018deep,ranjan2018light}.
Though effective enough for certain subjects, they suffer from performance degradation in unconstrained environments, \eg, free head motion and profile faces of subjects positioned further from the camera.
To track this issue, subsequent studies endeavor to construct datasets~\cite{eth,gaze360,gazecapture,eyediap} for gaze estimation in more physically unconstrained settings. 
Though they employed various methods to simulate real-world scenarios, such as using panoramic cameras to record multiple participants at once~\cite{gaze360} or multi-view photogrammetry to simulate gaze variations under extreme head poses~\cite{eth}, these approaches still rely on pre-defined assumptions that inherently simplify real-world complexity, and remain difficult to scale compared to web-crawled~\cite{CASIA-WebFace}, crowd-sourced~\cite{gazecapture} or synthetic data~\cite{FaceSynthetics}.


\noindent\textbf{Cross-domain Gaze Estimation.} 
The scarcity of diverse \textit{labeled training data} in appearance-based gaze estimation leads current fully-supervised methods to achieve strong \textit{within-domain} performance but suffer from poor generalization in \textit{cross-domain} scenarios. 
To address this challenge, recent efforts for gaze estimation can be categorized into two paradigms: domain adaptation and domain generalization.
Domain adaptation approaches primarily try to minimize the domain discrepancy between source domain and known target domain via strategies, \eg, adversarial learning~\cite{gaze360,wang2019generalizing}, collaborative learning~\cite{liu2021generalizing}, contrastive learning~\cite{wang2022contrastive}, and consistency learning~\cite{bao2022generalizing,hisadome2024rotation}. 
In contrast, recent endeavors in domain generalization address a more realistic scenario without access to target samples, focusing on learning domain-invariant features through methods, \eg, self-adversarial learning to preserve gaze information~\cite{cheng2022puregaze} or data augmentation based on gaze-irrelevant factors~\cite{xu2023learning}. 
However, given the inherent diversity of face images (\eg, illumination, head orientation, and eye occlusion), these methods remain constrained by their reliance on the coverage of labeled source-domain data, which hinders their performance in the unconstrained real-world environments.


\noindent\textbf{Semi-supervised Learning.} 
The goal of semi-supervised learning (SSL) is to enhance model's performance under the limited availability of labeled data by leveraging unlabeled data. 
The two mainstream methods are entropy minimization~\cite{zhou2010semi,xie2020self} and consistency regularization~\cite{kim2022conmatch,wang2022freematch,yin2022semi,liang2023logic}.
The former is proposed based on the manifold assumption or the smoothness assumption, \ie, the model should output similar predictions regardless of input perturbations, which necessitates well-designed data augmentations based on the prior of specific tasks.
The latter encourages the model itself to output confident predictions on unlabeled data, leading to the main problem of SSL: \textit{how to efficiently select high-quality pseudo labels?} 
For classification tasks, FixMatch~\cite{sohn2020fixmatch} uses a fixed confidence threshold to filter out uncertain samples, while FlexMatch~\cite{zhang2021flexmatch} enhances this strategy with class-aware thresholds. 
Furthermore, SemiReward~\cite{li2023semireward} introduces a reward score based on cosine similarity between pseudo and groundtruth labels to evaluate the quality of pseudo labels.
Despite these advances, the SSL for gaze estimation still remain to be explored.






==> OminGaze_NeurIPS25_arxiv/sec/3_method.tex <==
\input{figs/overview}
\section{\textsc{OmniGaze}}
\label{sec::method}

%\noindent\textbf{Semi-supervised Training Pipeline.} 
\subsection{Semi-supervised Training Pipeline} 
We first formulate the semi-supervised framework in 3D gaze estimation.
Let $\mathcal{D}_L =\{x_{i}^l, y_{i}^l\}_{i=1}^{N_L}$ and $\hat{\mathcal{D}}_U=\{x_{j}^u\}_{j=1}^{N_U}$ denotes the labeled and unlabeled datasets, where $x_{i}^l$ and $x_{j}^u$ are the labeled and unlabeled face images, and $y_{i}^l$ is the 3D gaze ground truth label. 
To make use of all training data, the training pipeline of \textsc{OmniGaze} can be divided into three phases: 
\textbf{i) Pseudo-label generation}. 
% A teacher model $\theta_{T}$ is pre-trained on $\mathcal{D}_L$ via supervised learning, which is then applied to generate pseudo labels $y_{i}^u$ for $\mathcal{D}_U$.
Following previous self-training strategies~\cite{zhou2010semi,xie2020self}, a teacher model $\theta_{T}$ pre-trained on $\mathcal{D}_L$ via supervised learning is applied to generate pseudo labels $y_{j}^u$ for $\hat{\mathcal{D}}_U$;
\textbf{ii) Reward-driven pseudo-label selection}. To measure the reliability of continuous pseudo labels, a reward model is proposed to predict confidence scores, which are then used to filter out low-quality pseudo labels and reweight the contribution of high-quality samples in the loss calculation (\S\ref{sec::eva});
\textbf{iii) Student model self-training}. These high-quality samples along with labeled data are utilized to train a robust student model $h_{S}$ (\S\ref{sec::training}). A brief illustration of training pipeline is shown in Fig.~\ref{fig:overview}.
% ~\cite{rosenberg2005semi,zhou2010semi,xie2020self,pham2021meta}

\subsection{Learning Labeled Face Images} 
\noindent\textbf{Model Architecture.} 
Our gaze estimation model adopts a Vision Transformer (ViT) architecture~\cite{dosovitskiyimage}. 
Specifically, given an input image $x$, the model first extracts gaze representation via a transformer encoder, and then employs a lightweight MLP to regress the gaze direction $\hat{y}$ as yaw and pitch angles.

\noindent\textbf{Supervised Loss.} 
Following~\cite{cheng2022gaze,cheng2020coarse,fischer2018rt}, we adopt an angular loss to optimize our gaze estimator: 
\begin{equation}
\label{eq:sup}
\mathcal{L}^{\text{s}} = \frac{1}{N_L} \sum\nolimits_{i=1}^{N_L} \|\hat{y} - y_i^l \|_2,
\end{equation}
where $\hat{y}=h_T(x)$ is the estimation result.


\subsection{Unleashing the Power of Unlabeled Face Images}
\label{sec::unlabel}
\noindent\textbf{Unlabeled Face Image Collection.} 
Due to impoverished labeled data, current gaze estimators struggle to generalize to diverse real-world conditions, \eg, different facial appearance, extreme head poses, varying lighting conditions, and broader gaze distributions. 
To learn robust gaze representations, we attempt to harness the power of large-scale unlabeled face images, which are widely available through online repositories and publicly curated datasets~\cite{CelebA,vggface2,FaceSynthetics,SFHQ_T2I,xie2022vfhq,CASIA-WebFace} originally designed for facial analysis tasks.
Concretely, we compile face images from six public datasets to construct a large-scale unlabeled dataset compassing over 1.4 million images, which covers diverse head poses, lighting conditions, appearance, \emph{etc}. 
Table~\ref{tab:datasets} provides a detailed breakdown of this dataset.

\noindent\textbf{Pseudo-label Generation.}
Given an unlabeled dataset, we first developed a high-performing teacher model to automatically generate pseudo gaze labels.
Specifically, we make full use of existing labeled datasets to train this teacher model $h_T$ in a supervised manner. 
Then, we utilize $h_T$ to assign pseudo gaze labels on unlabeled images:
\begin{equation}
    \mathcal{D}_U = \{({x}_{j}^u, {y}_{j}^u) | y_{j}^{u}=h_T(x_{j}^{u}),  {x}_{j}^{u} \in \hat{\mathcal{D}}_U\}_{j=1}^{N_U},
\end{equation}
where $\mathcal{D}_U$ is the pseudo labeled dataset. Then we combine the labeled dataset and pseudo labeled dataset as a new training dataset $\mathcal{D}=\mathcal{D}_{L}\cup\mathcal{D}_{U}$ to jointly train a student model $h_S$.


\noindent\textbf{Pseudo-label Selection.}
Pseudo-labels generated by teacher models pre-trained on limited annotations are susceptible to confirmation bias. 
The effective utilization of \textit{noisy pseudo-labels} during training remains a persistent challenge in self-training paradigms. Prior research~\cite{sohn2020fixmatch,zhang2021flexmatch} has predominantly addressed this by filtering out low-quality pseudo-labels through dynamic or handcrafted thresholding strategies.
Though effective, these strategies are oriented for classification tasks while ill-suited for regression tasks like gaze estimation, where 3D gaze labels are continuous signals.
In this work, we accompany the student model $h_S$ with an auxiliary reward model $h_G$ that generates confidence scores to assess the reliability of pseudo-gaze labels.
By learning to distinguish between reliable and unreliable pseudo labels, $h_G$ can select high-quality samples from $\mathcal{D}_U$, thereby enhancing the utilization of unlabeled data and improving the efficacy of self-training for the student model.



\subsection{Empowering Reward Model with Multimodal Cues} 
\label{sec::eva}
Our reward model $h_G$ (\cf~Fig.~\ref{fig:overview}b) evaluates the reliability of pseudo labels by reasoning of multimodal cues: geometric gaze directions, visual feature, and semantic context.
By leveraging these cues, $h_G$ can capture the nuanced and context-dependent nature of gaze for robust confidence assessments.

\input{tabs/dataset_detail}
\noindent\textbf{Multimodal Cues Integration.}
To improve the generalization capability of the reward model for in-the-wild samples, we integrate multimodal cues, \eg, visual and linguistic cues, into the reward model, enabling it to distinguish visually similar but semantically different gaze patterns. 
\textbf{First}, we extract the visual cues by encoding the input image ${x}_{k} \in\mathcal{D}$ via the visual encoder of CLIP~\cite{radford2021learning}:
\begin{equation}
\small
\label{eq::visual}
    \bm{f}_{k}^{\text{v}} \!=\![\bm{f}_{\text{cls}}^{\text{v}}, \bm{f}_{1}^{\text{v}}, \bm{f}_{2}^{\text{v}}, \cdots, \bm{f}_{M}^{\text{v}}] \!=\! \texttt{MLP}(\texttt{Encoder}_\text{v}({x}_{k} )),
\end{equation}
where $M$ denotes the number of patch in the image.
\textbf{Second}, we further obtain the linguistic descriptions by questioning MLLMs, \eg, InstructBLIP~\cite{dai2023instructblipgeneralpurposevisionlanguagemodels}, on the input image with a pre-defined prompt: \textit{In 3D space, where is the person looking, including details about horizontal (left/right) direction, vertical (up/down) direction, and forward/backward relative to the viewer?}
Then, these descriptions are converted into linguistic embeddings $\bm{f}_{k}^{\text{t}}$ via the text encoder of CLIP.
Finally, we adopt cross-attention to aggregate $\bm{f}_{k}^{\text{v}}$ and $\bm{f}_{k}^{\text{t}}$, resulting in an semantic-aware gaze representation:
\begin{equation}
\small
\label{eq:mva_aggregate}
    \hat{\bm{f}}_{k}^{\text{v}} = \texttt{AvgPool}(\texttt{LN}(\texttt{CrossAttn}(\bm{f}_{k}^{\text{v}},\bm{f}_{k}^{\text{t}})),
\end{equation}
where $\texttt{AvgPool}$ is the average pooling. $\texttt{LN}$ is the standard layer normalization. $\texttt{CrossAttn}$ denotes the standard cross-attention operation, where visual features $\bm{f}_{k}^{\text{v}}$ is the query, and text features $\bm{f}_{k}^{\text{t}}$ is the key and value. As such, our reward model can dynamically attend to relevant semantic cues when interpreting visual features,  enhancing its ability to disambiguate subtle gaze variations. 
We provide more examples for generating scene-specific gaze descriptions in the Appendix.


\noindent\textbf{Reward Model as Scorer.}
Given a pseudo label $y_k=(\theta_{k},\psi_{k})$, we first interpolate it into a 3D direction vector. 
Compared to angular representations such as yaw and pitch, 3D direction vectors provide a more expressive and continuous formulation for modeling gaze behavior, which facilitates more precise alignment with semantic-aware gaze representations.
Specifically, we convert the pseudo gaze label into a 3D direction vector $\bm{v}_k$ using a Spherical-to-Cartesian coordinate transformation:
\begin{equation}
\small
\label{eq:inter}
    \bm{v}_k = [\cos(\psi_{k}) \cdot \sin(\theta_{k}), \cos(\psi_{k}), \cos(\psi_{k}) \cdot \cos(\theta_{k})].
\end{equation}
% 3D gaze vecotrs serve as geometry-aware targets that complement visual features during reward modeling, enhancing the model's ability to assess subtle gaze behaviors.
Leveraging the obtained semantic-aware gaze representation $\hat{\bm{f}}_k^{\text{v}}$ and 3D gaze vector $\bm{v}_k$, the reward model predicts confidence scores via a cross-attention followed by an MLP:
\begin{equation}
\small
\label{eq:int}
    \hat{r}_k = \texttt{Sigmoid}(\texttt{MLP}(\texttt{CrossAttn}(\hat{\bm{f}}_k^{\text{v}},\bm{v}_k))),
\end{equation}
where $\hat{r}_k\!\in\![0,1]$ and $\texttt{Sigmoid}$ denotes the Sigmoid function.
Such confidence score allows the reward model to assess the consistency between visual appearance, semantic cues, and gaze labels. 
To further strengthen the evaluation capability of reward model, we feed the confidence score $\hat{r}_k$ and the cosine similarity score (between the student model prediction $\hat{{y}}_{k}$ and the pseudo label ${y}_{k}$) into a label scorer implemented via a lightweight MLP to obtain final confidence scores $r_k \!\in\![0,1]$, yielding a holistic and reliable measure of pseudo-label quality:
\begin{equation}
\small
\label{eq:final}
r_k = \texttt{Sigmoid}(\texttt{MLP}([(\hat{r}_k, \text{sim}(\hat{{y}}_{k}, {y}_{k})])).
\end{equation}
%These holistic confidence scores are then utilized to measure whether the given label ${y}_{i}$ belongs to the ground-truth label set $\mathcal{D}^{\text{l}}$ or the pseudo-label set $\mathcal{D}^{\text{u}}$. 
These confidence scores are then utilized to filter out unreliable samples and reweight high-quality ones (see \S\ref{sec::training}), thus enhancing the stability and effectiveness of student model self-training.



\subsection{Training with Pseudo Labels}
\label{sec::training}
%After predicting confidence scores $\{r_{j}\}_{1}^{B}$ for a batch of  samples from combination dataset $\mathcal{D}=\mathcal{D}^{\text{l}} \cup \mathcal{D}^{\text{u}}$, we jointly optimize the rewarder and the student model in an online self-training framework.

\noindent\textbf{Training of Reward Model $h_G$.} We train reward model $h_G$ by jointly using the labeled and unlabeled dataset (\ie, $\mathcal{D}_L$ and $\mathcal{D}_U$), where we treat ground-truth gaze labels of labeled data as trust pseudo-labels. 
Formally, given confidence scores $\{r_{k}\}_{k=1}^{N_L+N_U}$ for $\mathcal{D}_L$ and $\mathcal{D}_U$, the reward model $h_G$ is supervised via a binary classification loss:
\begin{equation}
\small
\mathcal{L}^{\text{g}} = \sum\nolimits_{k=1}^{N_L+N_U} - (c_{k} \log(r_{k}) + (1 - c_{k}) \log(1 - r_{k})),
\end{equation}
where $c_{k} \in \{0, 1\}$ is a binary observability mask indicating the label source. Specifically,  $c_{k}\!=\! 1$  denotes that  $y_k$  is a ground-truth label, while  $c_k = 0 $ indicates that  $y_k$  is a pseudo label. By this means, the reward model gradually learns to distinguish between reliable and unreliable pseudo labels.

\noindent\textbf{Training of Student Model $h_S$.}
Meanwhile, our student model $h_S$ receives the confidence scores from the reward model $h_G$ for $\mathcal{D}_U$, which indicate the reliability of the corresponding pseudo labels.
These scores are used to modulate the learning  of the student model $h_S$ in two ways: \textbf{i}) filtering out low-confidence pseudo labels (\ie, $r_j \!<\! \tau$), and \textbf{ii}) adaptively reweighting the contribution of the remaining pseudo labels.
In other words, the reward model $h_G$ guides the student model to attach more attention to correct labels and ignore erroneous labels.
Formally, given $\mathcal{D}_U = \{x_{j}^{u}, y_{j}^{u}\}_{j=1}^{N_U}$ and corresponding confidence scores $\{r_{j}\}_{j=1}^{N_U}$, the unsupervised loss on unlabeled data can be defined as:  
\begin{equation}
\small
\label{eq:unsup}
    \mathcal{L}^{\text{u}} = \sum\nolimits_{j=1}^{N_U} \mathbbm{1}[r_j \ge \tau] \cdot r_j \cdot \| h_S(x_j^u)- y_j^u\|_2,
\end{equation}
where  $\mathbbm{1}[\cdot]$ is the indicator function for threshold filtering, and $\tau\!=\!0.5$ is a confidence threshold.
Specifically, if $h_G$ considers a pseudo label unreliable (\ie, $0 \!<\! r_j \!<\! 0.5$), the unsupervised loss $\mathcal{L}^{\text{u}}$ encourages  $h_S$  to increase its prediction gap from that pseudo label. In contrast, when $h_G$ highly trusts a pseudo label (\ie, $r_j \!\to\! 1$), $\mathcal{L}^{\text{u}}$ enforces stronger alignment between the student prediction and pseudo label. 
We also explored confidence-based soft weighting $\alpha\!\in\![0,1]$ for labeled samples, but it yielded limited practical benefits, leaving deeper analysis for future work. 
Finally, \textbf{overall training objective} of the student model $h_S$ is  an average combination of $\mathcal{L}^{\text{s}}$ (Eq.~\ref{eq:sup}) and $\mathcal{L}^{\text{u}}$ (Eq.~\ref{eq:unsup}).
%\noindent\textbf{Overall Objective.} Finally, tthe student model $h_S$ is supervised with an average combination of $\mathcal{L}^{\text{s}}$ (Eq.~\ref{eq:sup}) and $\mathcal{L}^{\text{u}}$ (Eq.~\ref{eq:unsup}).

\noindent\textbf{Pseudo-label Update Strategy.}  
To ensure training stability and robustness, we adopt a periodic pseudo-label update strategy, where the frozen teacher model's parameters are periodically refreshed with the student model's weights every $K$ epochs to regenerate pseudo-labels (ablation study in Table~\ref{tab::update} of Appendix). This interval mitigates the risk of early-stage overfitting to noisy labels while allowing the student model to progressively benefit from improved predictions over time.
% \section{\textsc{OmniGaze}}
% \label{sec::method}
% \noindent\textbf{Semi-supervised Training Pipeline.} 
% We utilize both labeled and large-scale unlabeled training data to generalize gaze estimation in the wild. Formally, the labeled and unlabeled datasets are dentoed as $\mathcal{D}^{\text{l}} =\{x_{i}^{\text{l}}, y_{i}^{\text{l}}\}_{i=1}^{M}$ and $\hat{\mathcal{D}}^{\text{u}}=\{x_{j}^{\text{u}}\}_{j=1}^{N}$ respectively, where $x_{i}^{\text{l}}$ and $x_{j}^{\text{u}}$ are input face images, and $y_{i}^{\text{l}}=(\theta_{i}^{\text{l}},\phi_{i}^{\text{l}})\!\in \!\mathbb{R}^2$ is the 3D gaze (\ie, yaw and pitch) label, which exhibits continuous properties. To make use of all training data, overall training pipeline of \textsc{OmniGaze} can be divided into three phases: \textbf{i) Pseudo-label generation}. We learn a teacher model $h^{\text{t}}$ on $\mathcal{D}^{\text{l}}$ in a supervised manner, and utilize $h^{\text{t}}$ to directly generate pseudo labels $y_{j}^{\text{u}}=h^{\text{t}}(x_{j}^{\text{u}})$ for $\hat{\mathcal{D}}^{\text{u}}$, results in a pseudo-labeled dataset  $\mathcal{D}^{\text{u}} = \{x_{j}^{\text{u}}, y_{j}^{\text{u}}\}_{=1}^{N}$ . Here we collect large-scale and diverse unlabeled training dataset, which accounts for crucial gaze estimation challenges such as facial appearance variations, extreme poses, and diverse lighting conditions (\S\ref{sec::unlabel}). \textbf{ii) Reward-driven pseudo-label selection}.  We propose a reward model $g$ to measure the reliability of pseudo gaze labels via confidence scores, and then use these scores to filter out low-quality pseudo gaze labels and adaptively reweigh the contribution of high-quality samples (\S\ref{sec::eva}).  \textbf{iii) Student model self-training}. We utilize selected unlabeled data with high-quality pseudo gaze labels along with labeled data to jointly train a robust student model $h^{\text{s}}$ (\S\ref{sec::training}). 
% A brief illustration of training pipeline is provided in Figure x.

% \subsection{Learning Labeled Images} 
% \noindent\textbf{Model Architecture.} Our gaze estimation model aims to predict 3D gaze directions in the form of yaw and pitch angles: $(\theta,\phi)$, from full-face images.
% Specifically, given an input image $x$, our student model $h^{\text{s}}$ first adopts an ViT~\cite{dosovitskiyimage} image encoder ($\texttt{Encoder}$)  to obtain gaze representation $\bm{f} \!\in \!\mathbb{R}^{D}$, and then employs a lightweight MLP head ($\texttt{MLP}$) to regress the gaze direction $y\!\in \!\mathbb{R}^{2}$: 
% \begin{small}
% \begin{equation}
%      y=h^{\text{s}}(x)=\texttt{MLP}(\texttt{Encoder}(x)).
% \end{equation}
% \end{small}
% \noindent\textbf{Supervised Loss.} 
% Given the labeled dataset  $\mathcal{D}^{\text{l}} =\{x_{i}^{\text{l}}, y_{i}^{\text{l}}\}_{i=1}^{M}$, the student model $h^{\text{s}}$ can be directly optimized via commonly used angular loss~\cite{cheng2022gaze,cheng2020coarse,fischer2018rt} in gaze estimation:
% \begin{small}
% \begin{equation}
% \mathcal{L}^{\text{s}} = \frac{1}{M} \sum\nolimits_{i=1}^{M} \| h^{\text{s}}(x_i^{\text{l}}) - y_i^{\text{l}} \|_2^2.
% \end{equation}
% \end{small}

% \subsection{Unleashing the Power of Unlabeled Facial Images}
% \label{sec::unlabel}
% \noindent\textbf{Unlabeled Facial Image Collection.} 
% Current gaze estimation models encounter significant challenges in generalizing to unseen face images under diverse real-world conditions, \eg, diverse facial appearance, extreme head poses, varying lighting conditions, and broader gaze distributions, due to impoverished labeled training data. 
% %Existing labeled training datasets are typically collected in environmental conditions, with limited gaze distributions.
% To learn robust gaze representations in the wild, we attempt to harness the power of large-scale unlabeled face images, which offer a rich diversity of natural gaze cues.
% Nowadays, large-scale unlabeled face images are readily accessible from the Internet or existing public datasets collected for face analysis. Furthermore, we can easily obtain pseudo gaze annotations of unlabeled data using a teacher model trained on labeled gaze datasets in one single forward pass. 
% % 
% Concretely, we collect face images from six public datasets to curate the large unlabeled dataset, which provides rich diversity in facial appearance, head poses, lighting conditions, and image resolutions. Table~\ref{tab:datasets} summarizes the details of our large-scale unlabeled gaze dataset, which contain more than 1.4M images in total.

% \noindent\textbf{Pseudo-label Generation.}
% Given our unlabeled dataset without any form of labels, we built a data engine, which require a well-performed teacher model to automatically generate pseudo gaze labels for each unlabeled image.
% Specifically, we collect about 0.9M labeled images from two public datasets (\ie, Gaze360~\cite{gaze360} and ETH-Xgaze~\cite{eth}) to learn such reliable teacher model  $h^{\text{t}}$ in a supervised manner. 
% %Note that we exclude several existing labeled gaze datasets (\eg, MPIIFaceGaze~\cite{zhang2017s}, EyeDiap~\cite{eyediap}, RT-Gene~\cite{fischer2018rt}) from the training dataset to ensure zero-shot evaluation on gaze estimation models.
% Then we utilize $h^{\text{t}}$ to assign pseudo gaze labels on unlabeled face images:
% \begin{small}
% \begin{equation}
%     \mathcal{D}^{\text{u}} = \{({x}_{j}^{\text{u}}, {y}_{j}^{\text{u}}) | y_{j}^{\text{u}}=h^{\text{t}}(x_{j}^{\text{u}}),  {x}_{j}^{\text{u}} \in \hat{\mathcal{D}}^{\text{u}}\}_{j=1}^N,
% \end{equation}
% \end{small}
% where $\mathcal{D}^{\text{u}}$ is the pseudo-label dataset. Then we combine the labeled dataset and pseudo labeled dataset as a new training dataset $\mathcal{D}=\mathcal{D}^{\text{l}}\cup\mathcal{D}^{\text{u}}$ to jointly train a student model $h^{\text{s}}$.

% \noindent\textbf{Pseudo-label Selection.}
% Though our method has gained partial performance improvement with such a self-training pipeline, there exist \textit{noisy pseudo-labels} during training, hindering the model from fully unlocking the potential of large-scale unlabeled data. 
% During training, such noisy pseudo gaze labels introduce misleading supervisory signals, causing the model to learn incorrect visual-gaze associations. In this way, these erroneous predictions are accumulated over time through such pipeline, leading to severe confirmation bias, \ie, overfitting to noise pseudo labels from the teacher model.
% To address the confirmation bias issue in self-training, many previous works filter out low-quality pseudo labels via dynamic or hand-crafted threshold-based pseudo labeling selection strategies.
% Though effective, these confidence-based label selection strategies are oriented for classification tasks while impractical for regression tasks like gaze estimation, where 3D gaze labels are continuous signals and lack confidence information.
% In this work, instead of relying on threshold-based pseudo-labeling strategies, we accompany the student model $h^{\text{s}}$ with an auxiliary reward model $g$, which judges the reliability of pseudo gaze labels independent of the gaze estimation. 
% By learning to distinguish between reliable and unreliable pseudo labels, $g$ can select high-quality pseudo labels from $\mathcal{D}^{\text{u}}$ to make more effective use of unlabeled data, thus guiding the self-training of the student model.

% \subsection{Empowering Reward Model with Multimodal Cues} 
% \label{sec::eva}
% Our reward model $g$ evaluates the reliability of pseudo labels by jointly reasoning over visual appearance, semantic context, and geometric gaze directions. By making full use of multimodal cues like humans, reward model captures the nuanced and context-dependent nature of gaze behaviors for accurate confidence assessments.

% \noindent\textbf{Reward Modeling.}
% Given a full-face image ${x}_{j} \in\mathcal{D}$, the initial visual features can be obtained from the visual encoder of CLIP, followed by a lightweight, learnable MLP:
% \begin{equation}
% \small
% \label{eq::visual}
%     \bm{f}_{j}^{\text{v}} \!=\![\bm{f}_{\text{cls}}^{\text{v}}, \bm{f}_{1}^{\text{v}}, \bm{f}_{2}^{\text{v}}, \cdots, \bm{f}_{M}^{\text{v}}] \!=\! \texttt{MLP}(\texttt{Encoder}_\text{v}({x}_{j} )),
% \end{equation}
% where $\texttt{Encoder}_\text{v}$ is frozen visual encoder of CLIP, $\texttt{MLP}$ denotes a learnable MLP, and $M$ denotes the number of patch in the image.

% To better capture the underlying geometry of gaze behavior, we interpolate the pseudo label $y_j=(\theta_{j},\phi_{j})$ (\ie, yaw and pitch) into a 3D direction vector. 
% Compared to angular representations such as yaw and pitch, 3D direction vectors provide a more expressive and continuous formulation for modeling gaze behavior, which facilitates more precise alignment with semantic-aware gaze representations.
% Specifically, we convert the pseudo gaze label into a 3D direction vector $\bm{v}_j$ using a Spherical-to-Cartesian coordinate transformation:
% \begin{equation}
% \small
% \label{eq:mva_aggregate}
%     \bm{v}_j = [\sin(\phi_{j}) \cdot \cos(\theta_{j}), \sin(\phi_{j}) \cdot \sin(\theta_{j}), \cos(\phi_{j})].
% \end{equation}
%  3D gaze vectors serve as geometry-aware targets that complement visual features during reward modeling, enhancing the model's ability to assess subtle gaze behaviors.

% \input{tabs/dataset_detail}
%  \noindent\textbf{Multimodal Cue Integration.}
% Though visual features effectively capture appearance cues, only relying on them may struggle to distinguish visually similar but semantically different gaze patterns, thus leading to inaccurate confidence assessments.
% To alleviate this, we further make full use of scene-specific gaze descriptions provided by Multimodal Large Language Models (MLLMs), \eg, structBLIP, to complement the semantic context that enhances the reasoning ability of the reward model.
% Specifically,  we straightforwardly prompt structBLIP with a question like ``In 3D space, where is the person looking, including details about vertical direction, and horizontal direction?'' and the full-face image. structBLIP's response provides detailed scene-specific gaze descriptions based on visual content and its statistical training on large corpus. Then the gaze descriptions are fed into the text encoder of CLIP to extract corresponding text embeddings $\bm{f}_{j}^{\text{t}}$.
% Next, we adopt cross-attention to aggregate $\bm{f}_{j}^{\text{v}}$ and $\bm{f}_{j}^{\text{t}}$, resulting in an semantic-aware gaze representation $\hat{\bm{f}}_{j}^{\text{v}}$:
% \begin{equation}
% \small
% \label{eq:mva_aggregate}
%     \hat{\bm{f}}_{j}^{\text{v}} = \texttt{AvgPool}(\texttt{LN}(\texttt{CrossAttn}(\bm{f}_{j}^{\text{v}},\bm{f}_{j}^{\text{t}})),
% \end{equation}
% where $\texttt{AvgPool}$ is the average pooling. $\texttt{LN}$ is the standard layer normalization. $\texttt{Cros sAttn}(\bm{Q},\bm{KV})$ denotes the standard cross-attention operation, where visual features $\bm{f}_{j}^{\text{v}}$ is the query, and text features $\bm{f}_{j}^{\text{t}}$ is the key and
% value. As such, our reward model can dynamically attend to relevant semantic cues when interpreting visual features,  enhancing its ability to disambiguate subtle gaze variations. 
% We provide more details for generating scene-specific gaze descriptions {\color{red}in the Appendix}.


% \noindent\textbf{Reward Model as Scorer.}
% With above obtained semantic-aware gaze representation $\hat{\bm{f}}^{\text{v}}$ and 3D gaze vector $\bm{v}_j$, we models their correlation via a cross-attention module and an MLP module, and then produce initial confidence score $\hat{r}_j\!\in\![0,1]$ through Sigmoid function:
% \begin{equation}
% \small
% \label{eq:mva_aggregate}
%     \hat{r}_j = \texttt{Sigmoid}(\texttt{MLP}(\texttt{CrossAttn}(\hat{\bm{f}}^{\text{v}},\bm{v}))),
% \end{equation}

% where $\texttt{Sigmoid}$ is the Sigmoid function. $\texttt{MLP}$ is a learnable MLP module. $\texttt{CrossAttn}$ denotes the standard cross-attention operation.
% Such confidence score allows the reward model to assess the consistency between visual appearance, semantic cues, and gaze labels. 
% To further strengthen the evaluation capability of reward model, we feed the confidence score $\hat{r}_j$ and the cosine similarity score (between the student model prediction $\hat{{y}}_{j}$ and the pseudo label ${y}_{j}$) into a lightweight MLP to obtain final confidence scores $r_j \!\in\![0,1]$, yielding a holistic and reliable measure of pseudo-label quality:
% \begin{equation}
% \label{eq::stu}
% \small
% r_j = \texttt{Sigmoid}(\texttt{MLP}([(\hat{r}_j, \text{sim}(\hat{{y}}_{j}, {y}_{j})])).
% \end{equation}
% %These holistic confidence scores are then utilized to measure whether the given label ${y}_{i}$ belongs to the ground-truth label set $\mathcal{D}^{\text{l}}$ or the pseudo-label set $\mathcal{D}^{\text{u}}$. 
% These confidence scores are then utilized to filter out unreliable samples and reweigh high-quality ones, thus enhancing the stability and effectiveness of student model self-training.

% \subsection{Training with Pseudo Labels}
% \label{sec::training}
% %After predicting confidence scores $\{r_{j}\}_{1}^{B}$ for a batch of  samples from combination dataset $\mathcal{D}=\mathcal{D}^{\text{l}} \cup \mathcal{D}^{\text{u}}$, we jointly optimize the rewarder and the student model in an online self-training framework.

% \noindent\textbf{Training of Reward Model  $g$.} We train reward model $g$ by jointly using the labeled and unlabeled dataset (\ie, $\mathcal{D}^{\text{l}}$ and $\mathcal{D}^{\text{u}}$), where we treat ground-truth gaze labels of labeled data as trust pseudo-labels. Formally, given confidence scores $\{r_{k}\}_{1}^{M+N}$ for $\mathcal{D}^{\text{l}}$ and $\mathcal{D}^{\text{u}}$, the reward model $g$ is supervised via a binary classification loss:
% \begin{equation}
% \small
% \mathcal{L}^{\text{g}} = \sum\nolimits_{k=1}^{M+N}- ( c_{k} \log(r_{k}) + (1 - c_{k}) \log(1 - r_{k})),
% \end{equation}
% where $c_{k} \in \{0, 1\}$ is a binary observability mask indicating the label source. Specifically,  $c_{k}\!=\! 1$  denotes that  $y_k$  is a ground-truth label, while  $c_k = 0 $ indicates that  $y_k$  is a pseudo label. By this means, the reward model gradually learns to distinguish between reliable and unreliable pseudo labels.

% \noindent\textbf{Training of Student Model $h^{\text{s}}$.}
% Meanwhile, our student model $h^{\text{s}}$ receives the confidence scores from the reward model $g$ for $\mathcal{D}^{\text{u}}$, which indicate the reliability of the corresponding pseudo labels.
% These scores are used to modulate the learning  of the student model \( h^{\text{s}} \) in two ways: \textbf{i}) filtering out low-confidence pseudo labels (\ie, \( r_j < \tau \)), and \textbf{ii}) adaptively reweighing the contribution of the remaining pseudo labels.
% In other words, the reward model $g$ guides the student model to attach more attention to correct labels and ignore erroneous labels.
% Formally, given $\mathcal{D}^{\text{u}} = \{x_{j}^{\text{u}}, y_{j}^{\text{u}}\}_{j=1}^{N}$ and corresponding confidence scores $\{r_{j}\}_{1}^{N}$, the unsupervised loss on unlabeled data can be defined as:  
% \begin{equation}
% \small
% \label{eq:mva_aggregate}
%     \mathcal{L}^{\text{u}} = \sum\nolimits_{j=1}^{M} \mathbbm{1}[r_j \ge \tau] \cdot r_j \cdot \| h^{\text{s}}(x_j^{\text{u}})- y_j^{\text{u}}\|_2^2 ,
% \end{equation}
% where  $\mathbbm{1}[\cdot]$ is the indicator function for threshold filtering, and $\tau=0.5$ is a confidence threshold.
% Specifically, if $g$ considers a pseudo label unreliable (\ie, $0 < r_j < 0.5$), the unsupervised loss $\mathcal{L}^{\text{u}}$ encourages the student model  $h^{\text{s}}$  to increase its prediction gap from that pseudo label. In contrast, when $g$ highly trusts a pseudo label (\ie, $r_j \to 1$), $\mathcal{L}^{\text{u}}$ enforces stronger alignment between the student prediction and the pseudo label. 
% Although we also explored applying a soft weighting factor $\alpha\!\in\![0,1]$ to labeled samples based on the confidence scores, we observe limited benefits in practice and leave further investigation to future work. Finally, the student model $h^{\text{s}}$ is supervised with an average combination of $\mathcal{L}^{\text{s}}$ and $\mathcal{L}^{\text{u}}$.

% \noindent\textbf{Pseudo-Label Update Strategy.}  
% To ensure training stability and robustness, we adopt a periodic pseudo-label update strategy, which regenerates pseudo labels for the unlabeled dataset $\mathcal{D}^{\text{u}}$ every $K$ epochs. 
% This interval mitigates the risk of early-stage overfitting to noisy labels while allowing the student model to progressively benefit from improved predictions over time.
%This interval prevents the student model from being misled by low-quality pseudo gaze labels in the early training phase, while also allowing the model to benefit from progressively improved predictions as training progresses.





% version 2
% 第一阶段 训练教师模型。伪标签生成; 
% \noindent\textbf{Semi-supervised Training Pipeline.} 
% \textsc{OmniGaze} utilizes both labeled and unlabeled gaze training data to facilitate generalizable gaze estimation. Formally, the labeled and unlabeled datasets are dentoed as $\mathcal{D}^{\text{l}} = \left\{x_{i}^{\text{l}}, y_{i}^{\text{l}}\right\}_{i=1}^{M}$ and $\hat{\mathcal{D}}^{\text{u}}=\left\{x_{j}^{\text{u}}\right\}_{j=1}^{N}$ respectively, where $x_{i}^{\text{l}}$ and $x_{j}^{\text{u}}$ are input face images, and $y_{i}^{\text{l}}=(\theta_{i}^{\text{l}},\phi_{i}^{\text{l}})\!\in \!\mathbb{R}^2$ is the 3D gaze (\ie, yaw and pitch) label, which exhibits continuous properties. To make use of all training data, overall training pipeline of \textsc{OmniGaze} can be divided into three phase: \textbf{i) Pseudo-label generation}. We learn a teacher model $h^{\text{t}}$ on $\mathcal{D}^{\text{l}}$ in a supervised manner, and utilize $h^{\text{t}}$ to directly generate pseudo-labels $y_{j}^{\text{u}}=h^{\text{t}}(x_{j}^{\text{u}})$ for $\hat{\mathcal{D}}^{\text{u}}$, results in a pseudo-labeled dataset  $\mathcal{D}^{\text{u}} = \left\{x_{j}^{\text{u}}, y_{j}^{\text{u}}\right\}_{=1}^{N}$ . Here we collect large-scale and diverse unlabeled training dataset, which accounts for crucial gaze estimation challenges such as facial appearance variations, extreme poses, and diverse lighting conditions (\S\ref{sec::data}). \textbf{ii) Evaluator-driven pseudo-label assessment}. We construct a new training dataset $\mathcal{D}=\mathcal{D}^{\text{l}} \cup \mathcal{D}^{\text{u}}$ with both labeled and pseudo-labeled samples, and devise a confidence evaluator  $g$  to measure the reliability of pseudo gaze labels via jointly reasoning over visual appearance, semantic context, and gaze labels (\S\ref{sec::eva}).   \textbf{iii) Pseudo-label selection for student model training}. We first filter out low-quality pseudo gaze labels and adaptively reweighs the contribution of high-quality samples based on confidence scores provided by the evaluator, and utilize selected unlabeled data with high-quality pseudo gaze labels along with labeled data to jointly train a robust student model $h^{\text{s}}$ (\S\ref{sec::training}). 
% A brief illustration of training pipeline is provided in Figure xx.
%\textbf{ii)} and \textbf{iii)} are iteratively repeated until $h^{\text{s}}$  converges on the validation set. 

% \subsection{Data Engine: Pseudo-label Generation for Unlabeled  Facial Images}
% \label{sec::data}
% 现实场景视线估计有什么挑战。 当前的
% 不同于之前的方法 我们强调大规模无标注数据
% \noindent\textbf{Unlabeled Facial Image Collection.} 
% Current gaze estimation models encounter significant challenges in generalizing to unseen face images under diverse real-world conditions, \eg, diverse facial appearance, extreme head poses, varying lighting conditions, and broader gaze distributions, due to impoverished labeled training data. 
% Existing labeled training datasets are typically collected in environmental conditions, with limited gaze distributions.
% To learn robust gaze representations in the wild, we attempt to harness the power of large-scale unlabeled face images, which offer a rich diversity of natural gaze cues.
% Nowadays, large-scale and diverse unlabeled face images are readily accessible from the Internet or existing public datasets collected for face analysis. Furthermore, we can easily obtain pseudo gaze annotations of unlabeled data using a a teacher model trained on labeled gaze datasets in one single forward pass. 
% % 
% Specifically, we collect face images from five large-scale public datasets to curate the large unlabeled gaze dataset, which provides a high level of diversity, covering a wide range of head poses, gaze directions, lighting conditions, appearance, and imaging environments. Table~\ref{tab:datasets} summarizes the details of our large-scale unlabeled gaze datasets, which contain more than 1.5M images in total.

%\noindent\textbf{Data Pre-processing.} 

% \noindent\textbf{Pseudo-label Generation via Reliable Teacher Model.}
% Given our unlabeled dataset without any form of labels, we built a data engine, which require a well-performed teacher model to automatically generate pseudo gaze labels for each unlabeled image.
% Thus, we collect about 0.9M labeled images from 2 public datasets (\ie, Gaze360~\cite{gaze360} and ETH-Xgaze~\cite{eth}) to learn such reliable teacher model  $h^{\text{t}}$ in a supervised manner. 
% Note that we exclude several existing labeled gaze datasets (\eg, MPIIFaceGaze~\cite{zhang2017s}, EyeDiap~\cite{eyediap}, RT-Gene~\cite{fischer2018rt}) from the training dataset to ensure zero-shot evaluation on gaze estimation models.
% Then we utilize the obtained teacher model $h^{\text{t}}$ to assign pseudo gaze labels on unlabeled face images:
% \begin{small}
% \begin{equation}
%     \mathcal{D}^{\text{u}} = \{({x}_{j}^{\text{u}}, {y}_{j}^{\text{u}}) | y_{j}^{\text{u}}=f(x_{j}^{\text{u}}),  {x}_{j}^{\text{u}} \in \hat{\mathcal{D}}^{\text{u}}\}_{j=1}^N,
% \end{equation}
% \end{small}
% where $\mathcal{D}^{\text{u}}$ is the pseudo-label dataset. Then we make use of the combination of the labeled dataset $\mathcal{D}^{\text{l}}$ and pseudo labeled dataset $\mathcal{D}^{\text{u}}$ to jointly train a student model $h^{\text{s}}$.
% 是否介绍一下初始化model

% \subsection{Challenges in Directly Using Pseudo-Label Facial Images} 
% \label{sec::challenge}
% 虽然直接利用伪标签数据和有标注数据联合训练取得了一定的效果。尽管如此，这样做并没有完全释放出伪标注数据的潜力。


% we overlook the limitations of these pseudo-label gaze data, thereby hindering the model from fully unlocking their potential. 
% 存在噪声伪标签 噪声为标签在这个任务中的不好

% We find that there exists \textit{noisy pseudo-label gaze data} during training. Gaze direction is a fine-grained and context-sensitive attribute that can be easily affected by head pose, occlusions, and lighting conditions. Thus,  certain gaze pseudo labels may deviate from true gaze labels due to the limited generalization ability of the teacher model. 
% During training, such noisy gaze labels introduce misleading supervisory signals, causing the model to learn incorrect visual-gaze associations. In this way, these erroneous predictions are accumulated over time through such pipeline, leading to severe confirmation bias, \ie, overfitting to noise pseudo labels from the teacher model.
% Thus, \textit{it becomes essential to assess the reliability of pseudo gaze labels and selectively incorporate high-confidence pseudo gaze labels into the training process to reduce the label noise.}

% To address the confirmation bias issue in self-training, many previous works filter out low-quality pseudo labels via dynamic or hand-crafted threshold-based pseudo labeling selection strategies.
% Though effective, these confidence-based label selection strategies are designed for classification tasks, where the model outputs class prediction probabilities.
% In contrast, in the gaze estimation task, gaze estimation algorithms directly predict  3D gaze labels, which are continuous signals and lack confidence information.
% Thus, it is challenging to select reliable pseudo gaze labels via confidence-based strategies for gaze estimation.
% In this work, instead of relying on confidence-based selection, we accompany the student model $h^{\text{s}}$ with an auxiliary pseudo-label confidence evaluator $g$, which judges the reliability of pseudo gaze labels independent of the gaze estimation. 
% By learning to distinguish between reliable and unreliable pseudo labels, $g$ can denoise the pseudo-labeled set to make more effective use of pseudo-labeled gaze data, thus guiding the self-training of the student model.

% \subsection{Confidence Evaluator: Pseudo-label Assessment for Unlabeled Data} 
% \label{sec::eva}
% % Our goal is to address the challenge of high-quality pseudo gaze label selection for self-training, where the continuous nature of 3D gaze labels renders traditional confidence-based selection strategies impractical.
% % Thus, we propose a confidence evaluator that predicts confidence scores of pseudo labels via jointly reasoning over visual appearance, semantic context, and gaze labels.
% % % 感觉需要先总写一下？
% % Such evaluator design aims to disambiguate subtle gaze variations for accurate confidence assessments.

% \noindent\textbf{Semantic-aware Gaze Representation = Visual Appearance + Scene-specific Gaze Descriptions.} Given a full-face image ${x}_{i} \in\mathcal{D}$, the initial visual features can be obtained from the visual encoder of CLIP, followed by a lightweight, learnable MLP:
% \begin{equation}
% \small
% \label{eq::visual}
%     \bm{f}^{\text{v}} \!=\![\bm{f}_{\text{cls}}^{\text{v}}, \bm{f}_{1}^{\text{v}}, \bm{f}_{2}^{\text{v}}, \cdots, \bm{f}_{M}^{\text{v}}] \!=\! \texttt{MLP}(\texttt{Encoder}_\text{v}({x}_{i} )),
% \end{equation}
% where $\texttt{Encoder}_\text{v}$ is frozen visual encoder of CLIP, $\texttt{MLP}$ denotes a learnable MLP, and $M$ denotes the number of patch in the image.
% Though visual features effectively capture appearance cues, only relying on them may struggle to distinguish visually similar but semantically different gaze patterns, thus leading to inaccurate confidence assessments.

% To alleviate this, we further make full use of scene-specific gaze descriptions provided by Multimodal Large Language Models (MLLMs), \eg, structBLIP, to complement the semantic context that enhances the reasoning ability of evaluator.
% Specifically,  we straightforwardly prompt MLLM with a question like ``In 3D space, where is the person looking, including details about vertical direction, and horizontal direction?'' and the full-face image ${x}_{i}$. MLLM's response provides detailed scene-specific gaze description $d_i$ based on visual content and its statistical training on large corpus. Then the gaze descriptions are fed into the text encoder of CLIP to extract corresponding text embeddings $\bm{f}^{\text{t}}$.
% Next, we adopt cross-attention to aggregate $\bm{f}^{\text{v}}$ and $\bm{f}^{\text{t}}$, resulting in an semantic-aware gaze representation:
% \begin{equation}
% \small
% \label{eq:mva_aggregate}
%     \hat{\bm{f}}^{\text{v}} = \texttt{AvgPool}(\texttt{LN}(\texttt{CrossAttn}(\bm{f}^{\text{v}},\bm{f}^{\text{t}})),
% \end{equation}
% where $\texttt{AvgPool}$ is the average pooling. $\texttt{LN}$ is the standard layer normalization. $\texttt{CrossAttn}(\bm{Q},\bm{KV})$ denotes the standard cross-attention operation, where visual features $\bm{f}^{\text{v}}$ is the query, and text features $\bm{f}^{\text{t}}$ is the key and
% value. As such, our confidence evaluator can dynamically attend to relevant semantic cues when interpreting visual features,  enhancing its ability to disambiguate subtle gaze variations. 
% We provide more details for generating scene-specific gaze descriptions {\color{red}in the appendix}.

% \noindent\textbf{Geometry-aware Gaze Label Interpolation.}
% To better capture the underlying geometry of gaze behavior, we interpolate the pseudo label $y_i$ (\ie, yaw and pitch) into dense 3D direction vectors. This geometry-aware interpolation provides detailed structural information about gaze, facilitating more accurate alignment between above semantic-aware gaze representations and gaze directions. 
% Specifically, we convert the pseudo gaze label into 3D direction vector using a spherical-to-Cartesian coordinate transformation:
% \begin{equation}
% \small
% \label{eq:mva_aggregate}
%     \bm{v} = [\sin(\phi) \cdot \cos(\theta), \sin(\phi) \cdot \sin(\theta), \cos(\phi)],
% \end{equation}
% where  $\theta$ is the yaw angle of pseudo gaze label $y_i$, $\phi$ is the pitch angle of pseudo gaze label $y_i$, and $\bm{v}$ denotes the 3D direction vector. By considering the continuous nature of gaze behavior, this interpolation ensures that the gaze direction vector more accurately reflects real-world gaze patterns, so as to improve the reliability of the pseudo-label evaluation.

% \noindent\textbf{Confidence Score Prediction.}
% With above obtained semantic-aware gaze representation $\hat{\bm{f}}^{\text{v}}$ and 3D gaze vector $v$, confidence evaluator  models their correlation via a cross-attention module and an MLP module, and then produce initial confidence score $\hat{r}\!\in\![0,1]$ through
% Sigmoid function:
% \begin{equation}
% \small
% \label{eq:mva_aggregate}
%     \hat{r} = \texttt{Sigmoid}(\texttt{MLP}(\texttt{CrossAttn}(\hat{\bm{f}}^{\text{v}},\bm{v}))),
% \end{equation}
% where $\texttt{Sigmoid}$ is the Sigmoid function. $\texttt{MLP}$ is a learnable MLP module. $\texttt{CrossAttn}$ denotes the standard cross-attention operation. Such confidence score allows the evaluator to assess the consistency between visual appearance, semantic cues, and gaze labels. 
% To further strengthen the evaluation capability of the evaluator, we feed the initial confidence score $\hat{r}$ and the cosine similarity score (between the student model prediction $\hat{{y}}_{i}$ and the pseudo/true label ${y}_{i}$) into a lightweight MLP to obtain final confidence scores $r\!\in\![0,1]$, yielding a holistic and reliable measure of pseudo-label quality:
% \begin{equation}
% \small
% r_{i} = \texttt{Sigmoid}(\texttt{MLP}([(\hat{r}, \text{sim}(\hat{{y}}_{i}, {y}_{i}]))).
% \end{equation}
% These holistic confidence scores are then utilized to measure
%  whether the given label ${y}_{i}$ belongs to the ground-truth label set $\mathcal{D}^{\text{l}}$ or the pseudo-label set $\mathcal{D}^{\text{u}}$. Further, we make use of these confidence scores to filter unreliable samples and reweight high-quality ones during training, promoting more stable and effective self-training.

% \subsection{Training Strategy of \textsc{OmniGaze} via Labeled and Unlabeled Data}
% \label{sec::training}
% After predicting confidence scores $\{r_{j}\}_{1}^{B}$ for a batch of  samples from combination dataset $\mathcal{D}=\mathcal{D}^{\text{l}} \cup \mathcal{D}^{\text{u}}$, we jointly optimize the rewarder and the student model in an online self-training framework.

% \noindent\textbf{Training of Confidence Evaluator $g$.} We train the confidence evaluator by joint using labeled and unlabeled data, where we treat ground-truth gaze labels of labeled data as trusted pseudo-labels. Formally, given confidence scores $\{r_{i}\}_{1}^{B}$, the confidence evaluator is supervised via a binary classification loss:
% \begin{equation}
% \small
% \mathcal{L}_{\text{g}} = \sum\nolimits_{i=1}^{B}- \left( c_{i} \log(r_{i}) + (1 - c_{i}) \log(1 - r_{i}) \right),
% \end{equation}
% where $c_i \in \{0, 1\}$ is a binary observability mask indicating the label source. Specifically,  $c_i \!=\! 1$  denotes that  $y_i$  is a ground-truth label, while  $c_i = 0 $ indicates that  $y_i$  is a pseudo label. By this means, the evaluator gradually learns to distinguish between reliable and noisy pseudo labels.

% \noindent\textbf{Training of Student Model $h^{\text{s}}$.}
% % 
% Meanwhile, our student model $h^{\text{s}}$ receives the confidence scores from the evaluator $g$, which indicate the reliability of the corresponding pseudo labels.
% These scores are used to modulate the learning behavior of the student model \( h^{\text{s}} \) in two ways: (1) filtering out low-confidence pseudo labels (\ie, \( r_j < \tau \)), and (2) adaptively reweighting the contribution of the remaining pseudo-labeled samples according to their confidence.
% In other words, the evaluator $g$ guides the student model to attach more attention to correct labels and ignore erroneous labels.
% Formally, given $\mathcal{D}^{\text{l}} = \left\{x_{i}^{\text{l}}, y_{i}^{\text{l}}\right\}_{I=1}^{B^{\text{l}}}$  and $\mathcal{D}^{\text{u}} = \left\{x_{j}^{\text{u}}, y_{j}^{\text{u}}\right\}_{J=1}^{B^{\text{u}}}$, the optimization objective of student model $h^{\text{s}}$ can be defined as:  
% \begin{equation}
% \small
% \label{eq:mva_aggregate}
%     \mathcal{L}_{\text{s}} = \sum\nolimits_{i=1}^{B^{\text{l}}} \ell\left(h^{\text{s}}(x_i^{\text{l}}), y_i^{\text{l}}\right) +\sum\nolimits_{j=1}^{B^{\text{u}}} \mathbbm{1}[r_j \ge \tau] \cdot r_j \cdot \ell\left(h^{\text{s}}(x_j^{\text{u}}), y_j^{\text{u}}\right) ,
% \end{equation}
% where  $\ell(\cdot)$ is commonly used angular loss in gaze estimation. $\mathbbm{1}[\cdot]$ is the indicator function for threshold filtering, and $\tau=0.5$ is a confidence threshold.
% Specifically, if $g$ considers a pseudo label unreliable (\ie, $0 < r_i < 0.5$), the training objective $\mathcal{L}_{\text{s}}$ encourages the student model \( h^{\text{s}} \) to increase its prediction gap from that pseudo label. In contrast, when \( g \) highly trusts a pseudo label (\ie, $r_j \to 1$), $\mathcal{L}_{\text{s}}$ enforces stronger alignment between the student prediction and the pseudo label. 
% Although we also explored applying a soft weighting factor $\alpha\!\in\![0,1]$ to labeled samples based on the confidence scores from the evaluator, we observe limited benefits in practice and leave further investigation to future work.

% \noindent\textbf{Pseudo-Label Update Strategy.}  
% To ensure training stability and robustness, we adopt a periodic pseudo-label update strategy, which regenerates pseudo labels for the unlabeled dataset $\mathcal{D}^{\text{u}}$ every $K$ epochs. This interval prevents the student model from being misled by low-quality pseudo gaze labels in the early training phase, while also allowing the model to benefit from progressively improved predictions as training progresses.

==> OminGaze_NeurIPS25_arxiv/sec/4_experiment.tex <==
\section{Experiment}
\label{sec::experi}
\subsection{Experimental Settings} 
\noindent\textbf{Training.}
\textsc{OmniGaze} is trained with a batch size of 512. The training of \textsc{OmniGaze} can be divided into two stages: \textbf{i)} The teacher model is trained on labeled datasets for 50 epochs. We utilize the Adam optimizer~\cite{kingma2014adam} with an initial learning rate of $0.005$, and a weight decay of $0.05$. \textbf{ii)} We train the student model and reward model on both labeled and unlabeled data for 40 epochs with a base learning rate of $0.001$ and $0.0001$, respectively. %The unlabeled facial images are annotated by a best-performed teacher model with a ViT-L encoder. %We balance both labeled and unlabeled datasets in a minibatch to ensure each dataset accounts for an almost equal ratio.
Hyper-parameter $K$ is empirically set to 10. 

\noindent\textbf{Testing.} 
Following previous works~\cite{eth,cheng2020coarse,ververas20243dgazenet}, we use one input image scale of $224\times224$ without any data augmentation for the sake of fairness. 
Note that, during model deployment, our \textsc{OmniGaze} does not bring any change to network architecture of the student model or additional computation cost. The reward model $h_G$ is directly discarded after network training.

\noindent\textbf{Evaluation Metric.}
Following the conventions~\cite{xu2024gaze,liu2024test,palmero2018recurrent,fischer2018rt}, we use the angular error for evaluation, where lower values indicate better performance.

\subsection{\textsc{OmniGaze} as Generalized Gaze Estimator} 
\label{sec::in_cross}
% We first pretrain \textsc{OmniGaze} on our curated training dataset, and then fine-tune it on downstream gaze estimation tasks to examine \textsc{OmniGaze} as a promising weight initialization. We investigate the effectiveness of \textsc{OmniGaze} on two representative settings: 1) \textit{in-domain} gaze estimation, where the model is trained and evaluated on the same dataset, and 2) \textit{cross-domain} gaze estimation, where the model is trained on one dataset, but evaluated in an unseen one.
We first pretrain \textsc{OmniGaze} on our curated training dataset, and then fine-tune it on downstream gaze estimation tasks to examine \textsc{OmniGaze} as the weight initialization. We investigate the effectiveness of \textsc{OmniGaze} on two settings: 1) \textit{in-domain} gaze estimation, \ie, training and testing on the same dataset, and 2) \textit{cross-domain} gaze estimation, \ie, training on one dataset, testing on an unseen one. 
In this part, we approach our algorithm on ViT-B encoder pre-trained on ImageNet-21K dataset~\cite{ridnik2021imagenet}.

%\eg, Gaze360~\cite{gaze360}, but evaluated in an unseen dataset, \eg, MPIIFaceGaze~\cite{zhang2017s}. 
\begin{table}[t]
    \centering
    \caption{\small{\textbf{Quantitative in-domain gaze estimation results} (\S\ref{sec::in_cross}) on five benchmarks~\cite{zhang2017s,eyediap,fischer2018rt,gaze360,cheng2024you}.}}
    \resizebox{0.98\linewidth}{!}{ %< auto-adjusts font size to fill line
    \setlength{\tabcolsep}{4.5pt}
    \renewcommand\arraystretch{0.9}
         \begin{tabular}{rl||ccccc}
        \hline
         \thickhline \rowcolor{mygray}
        Method \!\!  && MPIIFaceGaze~\cite{zhang2017s}  & EyeDiap~\cite{eyediap} & RT-Gene~\cite{fischer2018rt} & Gaze360~\cite{gaze360} & IVGaze~\cite{cheng2024you} \\
        \hline\hline
            FullFace~\cite{zhang2017s}\!\!\!\! &\pub{CVPRW17} & 4.93  & 6.53 & 10.00 & 14.99 & 13.67 \\
            RCNN~\cite{palmero2018recurrent}\!\!\!\! &\pub{BMVC18} & 4.10  & 5.31 & 10.30 & 11.23 & - \\
        Gaze360~\cite{gaze360}\!\!\!\! &\pub{ICCV19} & 4.06  & 5.36 & 7.06 & 11.04 & 8.15 \\
        RT-Gene~\cite{fischer2018rt}\!\!\!\! &\pub{ECCV18} & 4.66  & 6.02 & 8.60 & 12.26 & - \\
        XGaze~\cite{eth}\!\!\!\! &\pub{ECCV20} & 4.80  & 6.50 & 12.00 & - & \underline{7.06} \\
        CANet~\cite{cheng2020coarse}\!\!\!\! &\pub{AAAI20} & 4.27  & 5.27 & 8.27 & 11.20 & - \\
        GazeTR~\cite{cheng2022gaze}\!\!\!\! &\pub{ICPR22} & 4.00  & 5.17 & \underline{6.55} & 10.62 & 7.33 \\
        AGE-Net~\cite{shi2024agent}\!\!\!\! &\pub{ICIP24} & \underline{3.61}  & \underline{4.78} & - & - & - \\
        3DGazeNet~\cite{ververas20243dgazenet}\!\!\!\! &\pub{ECCV24} & 4.00  & - & - & \underline{9.60} & - \\
        \hline
         %\textsc{OmniGaze}-Small\!\!\!\!&(Ours)& \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} \\
         \textsc{OmniGaze}\!\!\!\!&(Ours)& \textbf{2.97}\tiny{$\pm$0.09} & \textbf{4.07}\tiny{$\pm$0.15} & \textbf{5.40}\tiny{$\pm$0.21} & \textbf{9.12}\tiny{$\pm$0.11} & \textbf{6.72}\tiny{$\pm$0.15} \\
         %\textsc{OmniGaze}-Large\!\!\!\!&(Ours)& \textbf{x} & \textbf{x} & \textbf{x} & \textbf{x} & \textbf{x} \\
         \hline
        \end{tabular}
        }
    \label{table:within}
    \vspace{-10pt}
\end{table}


\noindent\textbf{Dataset.}  
We curate a comprehensive training dataset by combining labeled gaze datasets with six public unlabeled face datasets~\cite{CelebA,vggface2,FaceSynthetics,SFHQ_T2I,xie2022vfhq,CASIA-WebFace} 
%(\ie, CelebA~\cite{CelebA}, VGGFace2~\cite{vggface2},  FaceSynthetics~\cite{FaceSynthetics},  SFHQ-T2I~\cite{SFHQ_T2I}, VFHQ~\cite{xie2022vfhq} and CASIA-WebFace~\cite{CASIA-WebFace}) 
(Table~\ref{tab:datasets}).
%This curated training dataset provides rich diversity in facial appearance, head poses, lighting conditions, and image resolutions. 
Note that in \textit{in-domain} gaze estimation, labeled gaze datasets comprises ETH-XGaze~\cite{eth} along with specific evaluation training datasets; In \textit{cross-domain} gaze estimation, we only use source datasets as labeled gaze datasets. For evaluation, beyond the test split of Gaze360~\cite{gaze360}, we further assess \textsc{OmniGaze} on four widely used benchmarks: MPIIFaceGaze~\cite{zhang2017s}, EyeDiap~\cite{eyediap}, RT-Gene~\cite{fischer2018rt}, and IVGaze~\cite{cheng2024you}. 


%These testing datasets are kept unseen during training, facilitating zero-shot and cross-domain generalization evaluations. 

%\noindent\textbf{Network Architecture.}
%In this part, we approach our algorithm on ViT-B encoder pre-trained on ImageNet-21K dataset. The ViT encoder outputs the class token as gaze representation. Then we use an additional MLP module to regress the final gaze prediction from such gaze representation. 


\noindent\textbf{In-domain Gaze Estimation.} 
We first compare \textsc{OmniGaze} with top-leading solutions on five widely used gaze estimation benchmarks under the in-domain evaluation setup.%, where all methods follow the same officially divided train and test split. 
As shown in Table~\ref{table:within}, \textsc{OmniGaze} surpasses recent state-of-the-art gaze estimation algorithms by solid margins. In particular, it yields \textbf{0.64}$^\circ$, \textbf{0.71}$^\circ$, and \textbf{1.15}$^\circ$ reductions in angular error on MPIIFaceGaze~\cite{zhang2017s}, EyeDiap~\cite{eyediap}, and RT-Gene~\cite{fischer2018rt} respectively. It is particularly impressive considering the fact that the improvement is solely achieved by our semi-supervised training scheme, without any network architectural modification. Notably, we adopt the basic network design for in-domain gaze estimation, and we believe our results can be further enhanced if equipped with more advanced architectures.

\input{tabs/cross_domain}
\noindent\textbf{Cross-domain Gaze Estimation.} 
Next we investigate the cross-domain generalization of \textsc{OmniGaze} under the cross-domain setting. 
Like previous studies~\cite{xu2023learning,bao2024feature,yin2024clip,yin2024lg} that report results for models trained on ETH-XGaze~\cite{eth} or Gaze360~\cite{gaze360}, we evaluate \textsc{OmniGaze} trained on the same labeled gaze dataset for the sake of fairness. 
Table~\ref{table:crossdataset} reports our comparison results with SOTA domain-generalization methods on ETH-XGaze~\cite{eth} and Gaze360~\cite{gaze360}.
We can observe that  our training algorithm always improves generalization on any dataset.
This proves the effectiveness of making use of labeled datasets and large-scale diverse unlabeled datasets.
% \begin{table}[t]
%     \centering
%     \caption{\small{\textbf{Cross-domain comparison results} with SOTA methods on MPIIFaceGaze~\cite{zhang2017s} and EyeDiap~\cite{eyediap}. $\mathcal{D}_\mathrm{E}$, $\mathcal{D}_\mathrm{G}$, $\mathcal{D}_\mathrm{M}$, and $\mathcal{D}_\mathrm{D}$ denote  ETH-XGaze~\cite{eth}, Gaze360~\cite{gaze360}, MPIIFaceGaze~\cite{zhang2017s} and EyeDiap~\cite{eyediap} datasets.}}
%     \resizebox{0.7\linewidth}{!}{ %< auto-adjusts font size to fill line
%     \setlength{\tabcolsep}{4.5pt}
%          \begin{tabular}{rl|cccc}
%         \hline
%          \thickhline \rowcolor{mygray}
%         Method \!\!  && $\mathcal{D}_\mathrm{E} \rightarrow \mathcal{D}_\mathrm{M}$ & $\mathcal{D}_\mathrm{E} \rightarrow \mathcal{D}_\mathrm{D}$ & $\mathcal{D}_\mathrm{G} \rightarrow \mathcal{D}_\mathrm{M}$ & $\mathcal{D}_\mathrm{G} \rightarrow \mathcal{D}_\mathrm{D}$ \\ 
%         \hline
%             FullFace~\cite{zhang2017s}\!\!\!\! &\pub{CVPRW17} & 11.13 & 14.42 & 12.35 & 30.15 \\ 
%         CANet~\cite{cheng2020coarse}\!\!\!\! &\pub{AAAI20} & - & - & 27.13 & 31.41 \\
%         PureGaze~\cite{cheng2022puregaze}\!\!\!\! &\pub{AAAI22} &7.08 &7.48& 9.28 &9.32\\
%         RAT~\cite{bao2022generalizing}\!\!\!\! &\pub{CVPR22} &7.40 &6.91 &7.69 &7.08\\
%         Gaze-Consistent~\cite{xu2023learning}\!\!\!\! &\pub{AAAI23} & 6.50& 7.44& 7.55& 9.03\\
%         AGG~\cite{bao2024feature}\!\!\!\! &\pub{CVPR24} & 5.91 &6.75 &7.87& 7.9 \\
%         CLIP-Gaze~\cite{yin2024clip}\!\!\!\! &\pub{AAAI24} &  6.41 &7.51 &6.89& 7.06 \\
%         LG-Gaze~\cite{yin2024lg}\!\!\!\! &\pub{ECCV24} &6.45 &7.22 &6.83& 6.86 \\
%         \hline
%         %\textsc{OmniGaze}-Small\!\!\!\!&(Ours)& \textbf{} & \textbf{} & \textbf{} & \textbf{} \\
%           \textsc{OmniGaze}\!\!\!\!&(Ours)& \textbf{4.57} & \textbf{4.84} & \textbf{4.45} & \textbf{5.75} \\
%          %\textsc{OmniGaze}-Large\!\!\!\!&(Ours)& \textbf{} & \textbf{} & \textbf{} & \textbf{} \\
%         \bottomrule
%         \end{tabular}
%         }
%     \label{table:crossdataset}
% \end{table}


\subsection{\textsc{OmniGaze} as Automatic Data Engine} 
\label{sec::zeroshot}
A fundamental challenge in gaze estimation lies in the limited availability of diverse and well-annotated training data. To address this, we propose to leverage \textsc{OmniGaze} as a general-purpose \textit{automatic data engine}—a system capable of generating reliable gaze annotations for face images under diverse conditions. Thus, we comprehensively validate the zero-shot gaze estimation capability of \textsc{OmniGaze}, \ie,  directly estimating gaze directions on unseen datasets or in-the-wild images.

\noindent\textbf{Dataset.} 
% 先介绍训练数据集 然后介绍评估数据集的特点
We curate a comprehensive training dataset by combining two public labeled 3D gaze datasets (\ie, Gaze360~\cite{gaze360} and ETH-XGaze~\cite{eth}) with six public unlabeled face datasets (see  Table~\ref{tab:datasets} for more details), comprising over 2.4M data samples in total.
 We assess \textsc{OmniGaze} on four unseen gaze estimation benchmarks, \ie, MPIIFaceGaze~\cite{zhang2017s}, EyeDiap~\cite{eyediap}, RT-Gene~\cite{fischer2018rt}, and IVGaze~\cite{cheng2024you}. 
%More details of the utilized training and testing data are provided in Table xx.

\noindent\textbf{Network Architecture.}
In principle, our semi-spervised learning scheme can be applied into any feature encoder. In our experiments, we approach our algorithm on  ViT-S, ViT-B, and ViT-L encoder. 
%We remove the final classification layer and use the class token as gaze representation, which is then fed into a lightweight MLP to regress the 3D gaze direction.

% 性能和之前的非zero-shot媲美
\noindent\textbf{Quantitative Zero-shot Benchmark Evaluation.}
%Our goal is to estimate gaze directions for all face images, making zero-shot performance crucial.
Table~\ref{table:zeroshot} summarizes the zero-shot generalization comparison results on four representative unseen datasets\cite{zhang2017s,eyediap,fischer2018rt,cheng2024you}. 
Note that we also adopt certain powerful ViT-based models (DINO-B~\cite{caron2021emerging}, ViT-B~\cite{dosovitskiyimage}, and FaRL-B~\cite{zheng2022general}) as the gaze feature encoder to fine-tune on labeled datasets, and directly evaluate on unseen datasets. DINO-B and ViT-B have general semantic representations, while FaRL-B is designed for face analysis tasks. %and pre-trained on 20 M LAION-Face samples.
As seen, both with a ViT-B encoder, \textsc{OmniGaze} consistently outperforms other ViT-based models on diverse scenes, proving the high versatility of our algorithm. 
%Moreover, our ViT-S model (\ie, \textsc{OmniGaze}-Small), even outperforms other ViT-based models on several unseen datasets, \eg, xx,xx and xx. The performance advantage of these small-scale gaze estimation models demonstrates their great potential in computationally-constrained scenarios. 
It is also worth noting that, though previous SOTA methods in the first block uses the corresponding training images (\textit{not zero-shot anymore}), our \textsc{OmniGaze} is still evidently superior to them on certain datasets, \eg, \textbf{4.00}$^\circ \rightarrow$ \textbf{3.44}$^\circ$ on MPIIFaceGaze. This highlights the remarkable potential of our model as an automatic data engine.
%capable of delivering strong zero-shot generalization across diverse domains.

% 这里是否需要做dino？
\input{figs/visual}
\input{tabs/zero-shot}
\noindent\textbf{Qualitative Zero-shot Results.}
We visualize predicted gaze directions by \textsc{OmniGaze} and base model (\ie, train on labeled datasets and directly evaluate unseen datasets) on four unseen datasets in Fig.~\ref{fig:visual} (left). We observe that, after considering data scale-up and filtering out noisy pseudo labels, \textsc{OmniGaze}  demonstrates generalization improvements with a lower angular error on each dataset.   

\noindent\textbf{Qualitative Results in the Wild.}
In Fig.~\ref{fig:visual} (right), we provide additional qualitative results on in-the-wild images, to resemble the practical zero-shot application in real-world conditions. 
Compared to the base model trained only on labeled datasets, our \textsc{OmniGaze} can predict gaze direction accurately in unseen diverse environments, \eg, extreme head poses, challenging lighting conditions, and diverse appearances. 
We respectfully refer the reviewer to the appendix (\S\ref{sec::qualitative}) for more qualitative results.    

\subsection{Diagnostic Analysis}
\label{sec::ab}
For in-depth analysis, we conduct ablative studies using ViT-B encoder under zero-shot setting~(\S\ref{sec::zeroshot}).

\noindent\textbf{Key Component Analysis.}
In Table~\ref{tab::core}, we first examine the efficacy of essential components in our algorithm. The $1^{st}$ row reports the result of the baseline model, which only trains on labeled datasets. For $2^{nd}$ row, through jointly training on labeled datasets and large-scale diverse unlabeled data in a semi-supervised manner, we observe consistent and modest improvements against the baseline on each dataset (\eg, 8.45$^\circ\! \rightarrow\! $ \textbf{5.42}$^\circ$ on EyeDiap~\cite{eyediap}). This supports our claim that large-scale unlabeled face images provides significantly high level of data diversity, thus enhancing zero-shot generalization of our method. Furthermore, after assessing and filtering out low-quality pseudo-labels via the reward model, the performance boosts to \textbf{3.44}$^\circ$ and \textbf{4.31}$^\circ$ on  MPIIFaceGaze and EyeDiap, respectively. This suggests that scaling up datasets and further selecting high-quality samples can work in a collaborative manner, confirming the effectiveness of our overall algorithmic design.

\input{tabs/ab_study}
\begin{table}[t]
\centering
\captionsetup{font=small}\caption{\textbf{Comparison results with the same backbone} (\S\ref{sec::ab}) on MPIIFaceGaze~\cite{mpiiface}, EyeDiap~\cite{eyediap} and  RTGene~\cite{cheng2024you} under the in-domain setting.}
\label{tab::backbone}
\resizebox{0.8\linewidth}{!}{
\setlength\tabcolsep{7.5pt}
\renewcommand\arraystretch{1}
\begin{tabular}{l|c||ccc}
\thickhline
\rowcolor{mygray} Method & Backbone & MPIIFaceGaze~\cite{mpiiface} & EyeDiap~\cite{eyediap} & RT-Gene~\cite{cheng2024you} \\
\hline
\hline
FullFace~\cite{zhang2017s} & AlexNet & 4.93 & 6.53 & 10.00 \\
Gaze360~\cite{gaze360} & ResNet-18 & 4.06 & 5.36 & 7.06 \\
XGaze~\cite{eth} & ResNet-50 & 4.80 & 6.50 & 12.00 \\
CANet~\cite{cheng2020coarse} & ResNet-50 & 4.27 & 5.27 & 8.27 \\
GazeTR~\cite{cheng2022gaze} & ResNet-18 & 4.00 & 5.17 & 6.55 \\
AGE-Net~\cite{shi2024agent} & ResNet-34 & 3.61 & 4.78 & -- \\
3DGazeNet~\cite{ververas20243dgazenet} & ResNet-18 & 4.00 & -- & -- \\
\hline
\textsc{Baseline} & ResNet-18 & 4.48 & 5.56 & 7.45 \\
\textbf{OminGaze (Ours)} & ResNet-18 & \textbf{3.46} & \textbf{4.37} & \textbf{5.89} \\
\hline
\end{tabular}
}
\vspace{-10pt}
\end{table}
\noindent\textbf{Network Design for Reward Model.}
We investigate the impact of scene-specific gaze descriptions and gaze label interpolation (\cf~Eq.\ref{eq:inter}) in the reward model (\S\ref{sec::eva}), which is summarized in Table~\ref{tab::eva}. We construct a \textsc{Baseline} model that directly predicts confidence scores based on the visual appearance and gaze labels. First, upon aggregating visual appearance and scene-specific gaze descriptions, all datasets observe notable improvements (\eg, 4.52$^\circ \! \rightarrow\! $ \textbf{3.69}$^\circ$ on MPIIFaceGaze~\cite{mpiiface}). This verifies the effectiveness of learning semantic-aware gaze representation. Second, after interpolating gaze labels into 3D direction vectors, we also achieve significant angular error reductions, revealing the value of capturing the underlying geometry of gaze behaviors. Finally, our full reward model delivers the best performance across all datasets, validating the joint effectiveness of our network design.

\noindent\textbf{Pseudo-label Filtering Strategy.}
We further probe the influence of different pseudo-label filtering strategies (\S\ref{sec::training}). 
As outlined in Table~\ref{tab::filtering},  %in a standard semi-supervised manner without any pseudo-label filtering strategy, the base model can achieve $xx^\circ$ on xx and $xx^\circ$ on xx in terms of the angular error.
by filtering out low-quality pseudo-labels, the method has a slight improvement of \textbf{0.79}$^\circ$ and \textbf{0.40}$^\circ$ angle error on MPIIFaceGaze~\cite{mpiiface} and EyeDiap~\cite{eyediap}, respectively.
In addition, using confidence scores to reweight the importance of different samples, the model also exhibits improvements in angle error, achieving  \textbf{3.84}$^\circ$ and \textbf{4.78}$^\circ$ on MPIIFaceGaze and EyeDiap, respectively.
 Outstandingly, \textsc{OmniGaze} achieves the highest performance on all datasets by integrating both confidence-based pseudo-label filtering and reweighting.
The empirical evidence proves that our design facilitates gaze representation learning of the student model.
%our design--filtering out unreliable pseudo labels and reweighting the importance of different high-quality samples via confidence scores--that facilitates gaze representation learning of the student model.

\noindent\textbf{Student Prediction in Confidence Evaluation.}
To evaluate the contribution of student model and pseudo label prediction similarity $\text{sim}(\hat{{y}}_{k}, {y}_{k})$ in final scores $r_k$ (\cf~Eq.~\ref{eq:final}), we remove the similarity $\text{sim}(\hat{{y}}_{k}, {y}_{k})$ from the final confidence scores (\cf~Eq.~\ref{eq:int}) and report the results in Table~\ref{tab::sp}. The absence of additional information about gaze estimation results in a slight performance decline, suggesting that this can serve as a complementary cue for the assessment ability of the reward model.

\noindent\textbf{Comparison with Same Backbone.}
To ensure a fair comparison and address potential concerns regarding backbone capacity, we present additional experiments using the same lightweight ResNet-18 backbone as several SOTA methods~\cite{cheng2022gaze,shi2024agent,ververas20243dgazenet} under the in-domain setting.
The comparison results are summarized in Table~\ref{tab::backbone}. As shown, our \textsc{OmniGaze} achieves consistently better performance than both the baseline and existing SOTA methods (\eg, GazeTR~\cite{cheng2022gaze}, AGE-Net~\cite{shi2024agent}, and 3DGazeNet~\cite{ververas20243dgazenet}) when adopting the similar backbone architecture. This confirms that the improvements stem from our proposed semi-supervised learning strategies rather than model scales.

%\noindent\textbf{Unlabeled Data Size.}
% Finally we study the impact of the unlabeled data size in Fig. x.
% We randomly sample subsets from each component dataset to create 25\%, 50\%, and 75\% subsets of the full unlabeled data. Note that 0\% subsets means our  \textsc{OmniGaze} is trained only on labeled data without any unlabeled data. 
% When jointly training our \textsc{OmniGaze} on both labeled and unlabeled data, we observe that \textsc{OmniGaze} gains stable improvements (\ie, xxx) as the size of unlabeled data grows (\ie, 50\% subset).
% %When more that 75\% subset, further increasing unlabeled data size gives marginal performance gains. We speculate this is because our performance is primarily driven by data diversity, which appears sufficient at this scale. 
% This study confirms our motivation to making full use of large-scale and diverse unlabeled data for predicting gaze direction accurately across various domains.


% \subsection{Diagnostic Analysis}
% \label{sec::ab}
% \input{tabs/core_module}
% \noindent\textbf{Key Component Analysis.}
% In table~\ref{tab::core}, we first examine the efficacy of the essential components of our algorithm. The $1^{st}$ row reports the result of a baseline model, which trains on labeled datasets in a supervised manner. For $2^{nd}$ row, through jointly training on labeled datasets and large-scale diverse unlabeled data in a semi-supervised manner, we observe consistent and modest improvements against the baseline on each dataset (\eg, $xx^\circ \rightarrow xx^\circ$ on MPIIFaceGaze and $xx^\circ \rightarrow xx^\circ$ EyeDiap). This supports our claim that large-scale and diverse unlabeled face images provides significantly high level of data diversity, thus enhancing zero-shot generalization of gaze estimation models. Furthermore, after assessing and filtering out high-quality pseudo-labels via confidence evaluator, the performance boosts to $xx^\circ$ and $xx^\circ$ on  MPIIFaceGaze and EyeDiap, respectively. This suggests that scaling up dataset and further filter out high-quality samples of them is able to  work in a collaborative manner, confirming the effectiveness of our overall algorithmic design.

% \input{tabs/design_eva}
% \noindent\textbf{Network Design for Confidence Evaluator.}
% Then, we investigate the impact of scene-specific gaze descriptions and gaze label interpolation in the confidence evaluator, which is summarized in Table~\ref{tab::eva}. We construct a \textsc{Baseline} model that directly predicts confidence scores based on the visual appearance and gaze labels. First, upon aggregating visual appearance and scene-specific gaze descriptions via cross-attention, all datasets in zero-shot setting observe notable improvements (\eg, ). This verifies the effectiveness of learning semantic-aware gaze representation that guides the evaluator to disambiguate subtle gaze variations via visual appearance and semantic context. Second, after incorporating geometry-aware gaze label interpolation into \textsc{Baseline}, we achieve significant reductions in angular error of $xx^\circ$ on xx and $xx^\circ$ on xx, revealing the value to capture the underlying geometry of gaze behaviors. Finally, our full confidence evaluator delivers the best performance across all datasets, validating the joint effectiveness of our comprehensive network design for evaluator.

% \input{tabs/selection}
% \noindent\textbf{Pseudo-label Filtering Strategy.}
% We further probe the influence of different pseudo-label filtering Strategies under the zero-shot setting. 
% As outlined in Table~\ref{tab::selection},  in a standard semi-supervised manner without any pseudo-label filtering strategy, the base model can achieve $xx^\circ$ on xx and $xx^\circ$ on xx in terms of the angular error.
% By applying confidence-based pseudo-label filtering, the method has a slight improvement of $x^\circ$ and $x^\circ$ angle error on xx and xx, respectively.
% In addition, using confidence scores to reweigh the importance of different samples, the model exhibits improvements in angle error, achieving  $x^\circ$ and $x^\circ$ on xx and xx, respectively.
% Outstandingly, \textsc{OmniGaze} achieves the highest performance on all datasets by integrating both confidence-based pseudo-label filtering and reweighting.
% The empirical evidence proves our design--filtering out unreliable pseudo labels and reweighting the importance of different high-quality samples via confidence scores--that facilitates gaze representation learning of the student model.

% \noindent\textbf{Unlabeled Data Size.}
% Finally we study the impact of the unlabeled data size in Fig. x.
% We randomly sample subsets from each component dataset to create 25\%, 50\%, and 75\% subsets of the full unlabeled data. Note that 0\% subsets means our  \textsc{OmniGaze} is trained only on labeled data without any unlabeled data. 
% When jointly training our \textsc{OmniGaze} on both labeled and unlabeled data, we observe that \textsc{OmniGaze} gains stable improvements (\ie, xxx) as the size of unlabeled data grows (\ie, 50\% subset).
% When more that 75\% subset, further increasing unlabeled data size gives marginal performance gains. We speculate this is because our performance is primarily driven by data diversity, which appears sufficient at this scale. This study confirms our motivation to making full use of large-scale and diverse unlabeled data for predicting gaze direction accurately across various domains.


%  需要做更多的backbone

%核心模块消融

% 是否利用语义信息

% 角度不进行变换
% confidence的利用 只进行过滤,
% 引入student model的预测


% unlabeled data size

% evaluator可解释性的两张图

%参数量分析

==> OminGaze_NeurIPS25_arxiv/sec/5_conclusion.tex <==
\section{Conclusion}
In this work, we present \textsc{OmniGaze}, a novel semi-supervised framework to effectively generalize gaze estimation in the wild via harnessing the power of large-scale unlabeled data.
To achieve this, we carefully construct a diverse collection of unlabeled face images, varying in head poses, illumination conditions, facial appearances, \emph{etc}, and devise a reward model to filter out noisy pseudo labels in unlabeled data.
The reward model jointly reasons over visual appearance, semantic gaze context, and geometric gaze labels to predict confidence scores for accurate pseudo-label assessments.
Extensive empirical analysis demonstrates that \textsc{OmniGaze} sets new SOTAs on both in-domain and cross-domain settings, and also exhibits excellent zero-shot generalization ability.













==> OminGaze_NeurIPS25_arxiv/supp_figs/data_sample.tex <==
\begin{figure}[!t]
    \centering
   \includegraphics[width=1.0\textwidth]{supp_figs/data.pdf} 
   \put(-277, 322){\small {\cite{eth}}}
   \put(-277.6, 212.68){\small {\cite{vggface2}}}
    \put(-269.05, 107.3){\small {\cite{FaceSynthetics}}}
    \put(-282, 1.3){\small {\cite{cheng2024you}}}
    \put(-81.5, 322.05){\small {\cite{gaze360}}}
    \put(-79, 212.68){\small {\cite{SFHQ_T2I}}}
    \put(-84, 107.3){\small {\cite{xie2022vfhq}}}
    \put(-82.6, 1.3){\small {\cite{CelebA}}}
   \captionsetup{font=small}
\caption{Additional examples of each dataset(\S\ref{supp::diver}). Our curated training dataset (\ie, labeled datasets and large-scale unlabeled data) exhibits wide variability in terms of capturing environments (\eg, indoor, outdoor, synthetic, or in-vehicle scenes), facial appearance, lighting conditions, head poses, \emph{etc}.}
    \label{fig::sample}
\end{figure}

==> OminGaze_NeurIPS25_arxiv/supp_figs/gaze_des.tex <==
\begin{figure}[!t]
    \centering
   \includegraphics[width=1.0\textwidth]{supp_figs/gaze_description.pdf} 
   \captionsetup{font=small}
\caption{Examples of the generated scene-specific gaze descriptions along with face images (\S\ref{sec::descriptions}).}
    \label{fig::description}
\end{figure}

==> OminGaze_NeurIPS25_arxiv/tabs/ab_study.tex <==
\begin{table}[t!]
\makeatletter\def\@captype{table}\makeatother\captionsetup{font=small}\caption{\small\textbf{A set of ablative studies} (\S\ref{sec::ab}) on multiple unseen datasets (MG:  MPIIFaceGaze~\cite{mpiiface}, ED: EyeDiap~\cite{eyediap}, RG: RT-Gene~\cite{fischer2018rt}) under the zero-shot setting.}
        \centering
        \small
	%\hspace{-0.7em}
	\begin{subtable}
  {0.67\linewidth}
   \centering
   \resizebox{\textwidth}{!}{
\setlength\tabcolsep{3pt}
\renewcommand\arraystretch{0.95}
\begin{tabular}{ccc||ccc}
\thickhline
\rowcolor{mygray}   Labeled data & Unlabeled data & Pseudo-labels selection & MG      & ED      & RG  \\
\hline
\hline
$\checkmark$&& &6.17 &8.45 &20.73\\
$\checkmark$&$\checkmark$&  &4.97 & 5.42 &13.75\\
\arrayrulecolor{gray}\hdashline\arrayrulecolor{black}
$\checkmark$&$\checkmark$&$\checkmark$ &$\mathbf{3.44}$ &$\mathbf{4.31}$ &$\mathbf{9.09}$\\
\hline
\end{tabular}
	}
		%\setlength{\abovecaptionskip}{0.3cm}
		\setlength{\belowcaptionskip}{-0.0cm}
		\caption{\small{Core components in \textsc{OmniGaze}}}
		\vspace{-6px}
        \label{tab::core}
	\end{subtable}
        \hspace{-0.7em}     
        \begin{subtable}{0.33\linewidth}
         \centering
        \small
		\resizebox{\textwidth}{!}{
			\setlength\tabcolsep{2pt}
\renewcommand\arraystretch{0.95}
\begin{tabular}{l||ccc}
\thickhline
\rowcolor{mygray}
 Confidence score &  MG& ED & RG  \\ \hline  \hline
  \textit{w/o} reward    &  4.97 & 5.42 &13.75    \\  \arrayrulecolor{gray}\hdashline\arrayrulecolor{black}
    $\hat{r}_k$ (Eq.~\ref{eq:int}) & 3.71      & 4.68 & 9.96    \\ 
   $r_k$ (Eq.~\ref{eq:final}) \textbf{(Ours)} & $\mathbf{3.44}$   & $\mathbf{4.31}$   & $\mathbf{9.09}$      \\ \hline
\end{tabular}
}
		%\setlength{\abovecaptionskip}{0.3cm}
		\setlength{\belowcaptionskip}{-0.0cm}
		\caption{\small{Confidence score}}
		\vspace{-6px}
		\label{tab::sp}
	\end{subtable} \\
	\begin{subtable}{0.6\linewidth}
  \centering
        \small
		\resizebox{\textwidth}{!}{
			\setlength\tabcolsep{3pt}
\renewcommand\arraystretch{0.95}
\begin{tabular}{l||ccc}
\thickhline
\rowcolor{mygray}
 Evaluator Component &  MG& ED & RG  \\ \hline  \hline
  \textsc{Baseline}    &  4.52 & 5.19 &12.01    \\  \arrayrulecolor{gray}\hdashline\arrayrulecolor{black}
       + Scene-specific Gaze Descriptions \textit{only}  & 3.69      & 4.78 & 10.23    \\ 
   + 3D Direction Vector \textit{only}   & 4.03   & 4.93   & 10.56     \\ 
   \arrayrulecolor{gray}\hdashline\arrayrulecolor{black}
 Gaze Descriptions + 3D Direction Vector \textbf{(Ours)}  & $\mathbf{3.44}$      & $\mathbf{4.31}$ & $\mathbf{9.09}$     \\ \hline
\end{tabular}	}
		\setlength{\abovecaptionskip}{0.3cm}
		\setlength{\belowcaptionskip}{-0.0cm}
		\caption{\small{Network design for reward model}}
		\vspace{-0.6cm}
		\label{tab::eva}
	\end{subtable}
        \hspace{-0.7em}
	\begin{subtable}{0.4\linewidth}
  \centering
        \small
		\resizebox{\textwidth}{!}{
			\setlength\tabcolsep{3.3pt}
\renewcommand\arraystretch{0.97}
\begin{tabular}{cc||ccc}
\thickhline
\rowcolor{mygray}
Filtering &  Reweighting &  MG& ED & RG  \\ \hline  \hline
  &   &   4.97  & 5.42 & 13.75     \\  
      $\checkmark$ &  & 4.18      & 5.02 & 11.71    \\ 
   &  $\checkmark$ & 3.84   & 4.78   & 10.39      \\ 
   \arrayrulecolor{gray}\hdashline\arrayrulecolor{black}
$\checkmark$&  $\checkmark$ & $\mathbf{3.44}$      & $\mathbf{4.31}$ & $\mathbf{9.09}$     \\ \hline
\end{tabular}
		}
			\setlength{\abovecaptionskip}{0.3cm}
		\setlength{\belowcaptionskip}{-0.0cm}
		\caption{\small{Filtering strategy}}
		\vspace{-0.6cm}
		\label{tab::filtering}
	\end{subtable}
\vspace{-7pt}
\end{table}


==> OminGaze_NeurIPS25_arxiv/tabs/core_module.tex <==
\begin{table*}[!t]
\centering 
\vspace{-2pt}
\captionsetup{font=small}\caption{\textbf{Analysis of core components}~(\S\ref{sec::ab}) in \textsc{OminGaze} on MPIIFaceGaze~\cite{zhang2017s}, EyeDiap~\cite{eyediap} and  IVGaze~\cite{cheng2024you} within zero-shot setting.}
\vspace{-2pt}
\label{tab::core}
\setlength\tabcolsep{3pt}
\renewcommand\arraystretch{0.9}
\begin{tabular}{ccc||ccc}
\thickhline

\rowcolor{mygray}   Labeled data & Unlabeled data & Pseudo-labels selection & MG      & ED      & RG  \\
\hline
\hline
$\checkmark$&& &6.07 &6.47 &20.73\\
$\checkmark$&$\checkmark$&  &4.87 & 5.63 &13.75\\
\hline
$\checkmark$&$\checkmark$&$\checkmark$ &3.04 &4.31 &9.09\\
\hline
\end{tabular}
 }
\vspace{-9pt}
\end{table*}

==> OminGaze_NeurIPS25_arxiv/tabs/cross_domain.tex <==
\begin{wraptable}[12]{r}{0.62\textwidth}
\vspace{-11pt}
\centering
    \caption{\small{\textbf{Quantitative cross-domain gaze estimation results} (\S\ref{sec::in_cross}). $\mathcal{D}_\mathrm{E}$, $\mathcal{D}_\mathrm{G}$, $\mathcal{D}_\mathrm{M}$, and $\mathcal{D}_\mathrm{D}$ denote  ETH-XGaze~\cite{eth}, Gaze360~\cite{gaze360}, MPIIFaceGaze~\cite{zhang2017s} and EyeDiap~\cite{eyediap} datasets.}}
    \vspace{-4pt}
    \resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
    \setlength{\tabcolsep}{2.3pt}
         \begin{tabular}{rl||cccc}
        \hline
         \thickhline \rowcolor{mygray}
        Method \!\!  && $\mathcal{D}_\mathrm{E} \!\rightarrow\! \mathcal{D}_\mathrm{M}$ & $\mathcal{D}_\mathrm{E} \!\rightarrow\! \mathcal{D}_\mathrm{D}$ & $\mathcal{D}_\mathrm{G} \!\rightarrow\! \mathcal{D}_\mathrm{M}$ & $\mathcal{D}_\mathrm{G} \!\rightarrow\! \mathcal{D}_\mathrm{D}$ \\ 
        \hline\hline
            FullFace~\cite{zhang2017s}\!\!&\pub{CVPRW17} & 11.13 & 14.42 & 12.35 & 30.15 \\ 
        CANet~\cite{cheng2020coarse}\!\! &\pub{AAAI20} & - & - & 27.13 & 31.41 \\
        PureGaze~\cite{cheng2022puregaze}\!\! &\pub{AAAI22} &7.08 &7.48& 9.28 &9.32\\
        RAT~\cite{bao2022generalizing}\!\!&\pub{CVPR22} &7.40 &6.91 &7.69 &7.08\\
        Gaze-Consistent~\cite{xu2023learning}\!\! &\pub{AAAI23} & 6.50& 7.44& 7.55& 9.03\\
        AGG~\cite{bao2024feature}\!\! &\pub{CVPR24} &  \underline{5.91} &\underline{6.75} &7.87& 7.90 \\
        CLIP-Gaze~\cite{yin2024clip}\!\! &\pub{AAAI24} &  6.41 &7.51 &6.89& 7.06 \\
        LG-Gaze~\cite{yin2024lg}\!\!&\pub{ECCV24} &6.45 &7.22 &\underline{6.83}& \underline{6.86} \\
        \hline
        %\textsc{OmniGaze}-Small\!\!\!\!&(Ours)& \textbf{} & \textbf{} & \textbf{} & \textbf{} \\
          \textsc{OmniGaze}\!\!&(Ours)& \textbf{5.07}\tiny{$\pm$0.18} & \textbf{4.84}\tiny{$\pm$0.23} & \textbf{4.95}\tiny{$\pm$0.15} & \textbf{5.75}\tiny{$\pm$0.29} \\
         %\textsc{OmniGaze}-Large\!\!\!\!&(Ours)& \textbf{} & \textbf{} & \textbf{} & \textbf{} \\
        \bottomrule
        \end{tabular}
        }
    \label{table:crossdataset}
\end{wraptable} 

==> OminGaze_NeurIPS25_arxiv/tabs/dataset_detail.tex <==
\begin{table}[t]
\centering
\caption{\small{Key characteristics of unlabeled training datasets used in \textsc{OminGaze}. In total, our \textsc{OminGaze} is trained on labeled images and \textbf{1.4M unlabeled facial images} jointly.}}
\label{tab:datasets}
\resizebox{1\linewidth}{!}{
\setlength\tabcolsep{3pt}
\renewcommand\arraystretch{0.9}
\begin{tabular}{l||c|ccccc|c}
\thickhline
\rowcolor{mygray}
\textbf{Dataset}  & \textbf{Appearance Diversity} & \textbf{Scene} & \textbf{Illumination} & \textbf{Head Pose} & \textbf{Eye Occ.} & \textbf{Face Res.} & \textbf{Size} \\
\hline
% Gaze360\textsuperscript{\dag}~\cite{gaze360}         & Age, gender (natural)         & In/outdoor & Varied         & Wide range       & \ding{55}                    & Medium              & $\sim$172K \\
% ETH-XGaze\textsuperscript{\dag}~\cite{eth}      & Limited (lab-captured)        & Indoor      & Controlled       & Wide range      & \ding{55}                   & High                & $\sim$750K \\
CelebA~\cite{CelebA}          & Attributes, makeup, age       & Studio-like  & Controlled         & Mostly frontal            & \ding{55}                   & Low                 & $\sim$177K \\
VGGFace2~\cite{vggface2}        & Identity, age, ethnicity      & Real-world   & Varied  & Wide range                & \ding{51}                 & Varying             & $\sim$489K \\
FaceSynthetics~\cite{FaceSynthetics} & Synthetic with variation & Synthetic    & Controlled        & Wide range       &\ding{51}              & High & $\sim$86K \\
SFHQ-T2I~\cite{SFHQ_T2I}         & Broad demographic & Synthetic & Varied           & Wide range           & \ding{51}      & High                & $\sim$120K \\
VFHQ~\cite{xie2022vfhq}         & High-fidelity & Real-world        & Varied        & Wide range       & \ding{51}       & High           & $\sim$210K \\
WebFace~\cite{CASIA-WebFace} & Identity, ethnicity  & Indoor  &Controlled    & Mostly frontal            & \ding{55}                   & Medium       & $\sim$354K \\
\hline
\end{tabular}}
\vspace{-10pt}
\end{table}

 

 

==> OminGaze_NeurIPS25_arxiv/tabs/design_eva.tex <==
\begin{table*}[!t]
\caption{\small{Detailed analysis of network design for confidence evaluator  on MPIIFaceGaze~\cite{zhang2017s}, EyeDiap~\cite{eyediap} and  IVGaze~\cite{cheng2024you} within zero-shot setting.}}
\label{tab::eva}
\centering
\small
\resizebox{0.55\textwidth}{!}{
\setlength\tabcolsep{3pt}
\renewcommand\arraystretch{0.95}
\begin{tabular}{l|ccc}
\thickhline
\rowcolor{mygray}
 Evaluator Component &  MG& ED & RG  \\ \hline  \hline
  \textsc{Baseline}    &  4.42 & 5.39 &12.01    \\  \arrayrulecolor{gray}\hdashline\arrayrulecolor{black}
       + Scene-specific Gaze Descriptions \textit{only}  & 3.59      & 4.78 & 10.23    \\ 
   + Gaze Label Interpolation \textit{only}   & 3.93   & 5.13   & 10.56     \\ 
   \arrayrulecolor{gray}\hdashline\arrayrulecolor{black}
 Gaze Descriptions + Label Interpolation  \textbf{(Ours)}   & 3.04      & 4.31 & 9.09     \\ \hline
\end{tabular}} \vspace{-0.2cm}
\end{table*}

==> OminGaze_NeurIPS25_arxiv/tabs/selection.tex <==
\begin{table*}[!t]
\caption{\small{The impact of pseudo-label filtering Strategies  on MPIIFaceGaze~\cite{zhang2017s}, EyeDiap~\cite{eyediap} and  IVGaze~\cite{cheng2024you} within zero-shot setting.}}
\label{tab::selection}
\centering
\small
\resizebox{0.38\textwidth}{!}{
\setlength\tabcolsep{3pt}
\renewcommand\arraystretch{0.95}
\begin{tabular}{cc|ccc}
\thickhline
\rowcolor{mygray}
Filtering &  Rewighting &  MG& ED & RG  \\ \hline  \hline
  &   &   $4.57$  & $5.63$ & $13.05$     \\  
      $\checkmark$ &  & $3.98$      & $5.02$ & $11.75$    \\ 
   &  $\checkmark$ & $3.54$   & $4.78$   & $10.39$      \\ 
$\checkmark$&  $\checkmark$ & $3.04$      & $4.31$ & $9.09$     \\ \hline
\end{tabular}} \vspace{-0.2cm}
\end{table*}

==> OminGaze_NeurIPS25_arxiv/tabs/stu_pre.tex <==
\begin{table*}[!t]
\caption{\small{Detailed analysis of network design for confidence evaluator  on MPIIFaceGaze~\cite{zhang2017s}, EyeDiap~\cite{eyediap} and  IVGaze~\cite{cheng2024you} within zero-shot setting.}}
\label{tab::SP}
\centering
\small
\resizebox{0.33\textwidth}{!}{
\setlength\tabcolsep{3pt}
\renewcommand\arraystretch{0.95}
\begin{tabular}{l|ccc}
\thickhline
\rowcolor{mygray}
 Confidence score &  MG& ED & RG  \\ \hline  \hline
  \textit{w/o} rewarder    &  4.42 & 5.39 &12.01    \\  \arrayrulecolor{gray}\hdashline\arrayrulecolor{black}
    $\hat{r}$ (Eq. x) & 3.59      & 4.78 & 10.23    \\ 
   $r$ (Eq. x)   & 3.93   & 5.13   & 10.56      \\ \hline
\end{tabular}} \vspace{-0.2cm}
\end{table*}

==> OminGaze_NeurIPS25_arxiv/tabs/zero-shot.tex <==
\begin{table}[t]
    \centering
    \caption{\small{\textbf{Quantitative zero-shot generalization results} (\S\ref{sec::zeroshot})  on MPIIFaceGaze~\cite{zhang2017s}, EyeDiap~\cite{eyediap}, RT-Gene~\cite{fischer2018rt}, and IVGaze~\cite{cheng2024you}.  Note that all methods in the first block follow the in-domain evaluation. We provide three model scales, based on ViT-S (24.8M), ViT-B (97.5M), and ViT-L (335.3M), respectively.}}
    %for different purposes
    \resizebox{0.98\linewidth}{!}{ %< auto-adjusts font size to fill line
    \setlength{\tabcolsep}{5.2pt}
    \renewcommand\arraystretch{0.9}
         \begin{tabular}{rl|c||cccc}
        \hline
         \thickhline \rowcolor{mygray}
        Method \!\!  && Zero-shot &MPIIFaceGaze~\cite{zhang2017s}  & EyeDiap~\cite{eyediap} & RT-Gene~\cite{fischer2018rt} &  IVGaze~\cite{cheng2024you} \\
        \hline \hline
         \rowcolor{LightGray}   FullFace~\cite{zhang2017s}\!\!\!\! &\pub{CVPRW17}& \ding{55} & 4.93  & 6.53 & 10.00 &  13.67 \\
       \rowcolor{LightGray} Gaze360~\cite{gaze360}\!\!\!\! &\pub{ICCV19}& \ding{55}  & 4.06  & 5.36 & 7.06  & 8.15 \\
      % \rowcolor{LightGray} RT-Gene~\cite{fischer2018rt}\!\!\!\! &\pub{ECCV18}& \ding{55}  & 4.66  & 6.02 & 8.60 & - \\
       %\rowcolor{LightGray} GazeTR~\cite{cheng2022gaze}\!\!\!\! &\pub{ICPR22}& \ding{55}  & 4.00  & 5.17 & 6.55 &  7.33 \\
        \rowcolor{LightGray}CANet~\cite{cheng2020coarse}\!\!\!\! &\pub{AAAI20}& \ding{55}  & 4.27  & 5.27 & 8.27 &  - \\
        \rowcolor{LightGray}3DGazeNet~\cite{ververas20243dgazenet}\!\!\!\! &\pub{ECCV24} & \ding{55} & 4.00  & - & - &  - \\
        \hline
        DINO-B~\cite{caron2021emerging}\!\!\!\!&\pub{ICCV21} & \ding{51} & 6.52 & 8.50 & 21.09 &  19.82\\
         ViT-B~\cite{dosovitskiyimage}\!\!\!\!&\pub{ICLR21} & \ding{51} & 6.17 & 8.85&20.73 & 18.97 \\
         FaRL-B~\cite{zheng2022general}\!\!\!\!&\pub{CVPR22} & \ding{51} & 6.09 & 8.12 & 19.80 & 18.06 \\
        \hline
         \textsc{OmniGaze}-Small\!\!\!\!&(Ours)& \ding{51} & 3.70\tiny{$\pm$0.13} & 4.85\tiny{$\pm$0.21} & 10.02\tiny{$\pm$0.35} &  11.87\tiny{$\pm$0.29} \\
         \textsc{OmniGaze}-Base\!\!\!\!&(Ours)& \ding{51} & \textbf{3.44}\tiny{$\pm$0.10} & \textbf{4.31}\tiny{$\pm$0.12} & \textbf{9.09}\tiny{$\pm$0.21} & \textbf{10.81}\tiny{$\pm$0.27} \\
         \textsc{OmniGaze}-Large\!\!\!\!&(Ours)& \ding{51} & 3.03\tiny{$\pm$0.07} & 4.15\tiny{$\pm$0.14} & 9.01\tiny{$\pm$0.18} &  10.43\tiny{$\pm$0.20}\\
         \hline
        \end{tabular}
        }
    \label{table:zeroshot}
    \vspace{-10pt}
\end{table}

==> tabs/core_module.tex <==
\begin{table*}[!t]
\centering 
\vspace{-2pt}
\captionsetup{font=small}\caption{\textbf{Analysis of core components}~(\S\ref{sec::ab}) in \textsc{OminGaze} on MPIIFaceGaze~\cite{zhang2017s}, EyeDiap~\cite{eyediap} and  IVGaze~\cite{cheng2024you} within zero-shot setting.}
\vspace{-2pt}
\label{tab::core}
\setlength\tabcolsep{3pt}
\renewcommand\arraystretch{0.9}
\begin{tabular}{ccc||ccc}
\thickhline

\rowcolor{mygray}   Labeled data & Unlabeled data & Pseudo-labels selection & MG      & ED      & RG  \\
\hline
\hline
$\checkmark$&& &6.07 &6.47 &20.73\\
$\checkmark$&$\checkmark$&  &4.87 & 5.63 &13.75\\
\hline
$\checkmark$&$\checkmark$&$\checkmark$ &3.04 &4.31 &9.09\\
\hline
\end{tabular}
 }
\vspace{-9pt}
\end{table*}

==> tabs/design_eva.tex <==
\begin{table*}[!t]
\caption{\small{Detailed analysis of network design for confidence evaluator  on MPIIFaceGaze~\cite{zhang2017s}, EyeDiap~\cite{eyediap} and  IVGaze~\cite{cheng2024you} within zero-shot setting.}}
\label{tab::eva}
\centering
\small
\resizebox{0.55\textwidth}{!}{
\setlength\tabcolsep{3pt}
\renewcommand\arraystretch{0.95}
\begin{tabular}{l|ccc}
\thickhline
\rowcolor{mygray}
 Evaluator Component &  MG& ED & RG  \\ \hline  \hline
  \textsc{Baseline}    &  4.42 & 5.39 &12.01    \\  \arrayrulecolor{gray}\hdashline\arrayrulecolor{black}
       + Scene-specific Gaze Descriptions \textit{only}  & 3.59      & 4.78 & 10.23    \\ 
   + Gaze Label Interpolation \textit{only}   & 3.93   & 5.13   & 10.56     \\ 
   \arrayrulecolor{gray}\hdashline\arrayrulecolor{black}
 Gaze Descriptions + Label Interpolation  \textbf{(Ours)}   & 3.04      & 4.31 & 9.09     \\ \hline
\end{tabular}} \vspace{-0.2cm}
\end{table*}

==> tabs/selection.tex <==
\begin{table*}[!t]
\caption{\small{The impact of pseudo-label filtering Strategies  on MPIIFaceGaze~\cite{zhang2017s}, EyeDiap~\cite{eyediap} and  IVGaze~\cite{cheng2024you} within zero-shot setting.}}
\label{tab::selection}
\centering
\small
\resizebox{0.38\textwidth}{!}{
\setlength\tabcolsep{3pt}
\renewcommand\arraystretch{0.95}
\begin{tabular}{cc|ccc}
\thickhline
\rowcolor{mygray}
Filtering &  Rewighting &  MG& ED & RG  \\ \hline  \hline
  &   &   $4.57$  & $5.63$ & $13.05$     \\  
      $\checkmark$ &  & $3.98$      & $5.02$ & $11.75$    \\ 
   &  $\checkmark$ & $3.54$   & $4.78$   & $10.39$      \\ 
$\checkmark$&  $\checkmark$ & $3.04$      & $4.31$ & $9.09$     \\ \hline
\end{tabular}} \vspace{-0.2cm}
\end{table*}

==> tabs/stu_pre.tex <==
\begin{table*}[!t]
\caption{\small{Detailed analysis of network design for confidence evaluator  on MPIIFaceGaze~\cite{zhang2017s}, EyeDiap~\cite{eyediap} and  IVGaze~\cite{cheng2024you} within zero-shot setting.}}
\label{tab::SP}
\centering
\small
\resizebox{0.33\textwidth}{!}{
\setlength\tabcolsep{3pt}
\renewcommand\arraystretch{0.95}
\begin{tabular}{l|ccc}
\thickhline
\rowcolor{mygray}
 Confidence score &  MG& ED & RG  \\ \hline  \hline
  \textit{w/o} rewarder    &  4.42 & 5.39 &12.01    \\  \arrayrulecolor{gray}\hdashline\arrayrulecolor{black}
    $\hat{r}$ (Eq. x) & 3.59      & 4.78 & 10.23    \\ 
   $r$ (Eq. x)   & 3.93   & 5.13   & 10.56      \\ \hline
\end{tabular}} \vspace{-0.2cm}
\end{table*}
